Reduced-Space Interior Point Methods in Power Grid Problems

Due to critical environmental issues, the power systems have to accommodate a significant level of penetration of renewable generation which requires smart approaches to the power grid control. Associated optimal control problems are large-scale nonlinear optimization problems with up to hundreds of millions of variables and constraints. The interior point methods become computationally intractable, mainly due to the solution of large linear systems. This document addresses the computational bottlenecks of the interior point method during the solution of the security constrained optimal power flow problems by applying reduced space quasi-Newton IPM, which could utilize high-performance computers due to the inherent parallelism in the adjoint method. Reduced space IPM approach and the adjoint method is a novel approach when it comes to solving the (security constrained) optimal power flow problems. These were previously used in the PDE-constrained optimization. The presented methodology is suitable for high-performance architectures due to inherent parallelism in the adjoint method during the gradient evaluation, since the individual contingency scenarios are modeled by independent set of the constraints. Preliminary evaluation of the performance and convergence is performed to study the reduced space approach.

==> 02IPM.tex <==
%The document is based on \cite{IPOPT2006} and \cite{ipoptThesis}, partly containing copy-paste sections and equations. The additional value of this summary is that it considers more general NLP problem including inequality constraints and provides extensive description of certain topics (barrier parameter, warm start, inertia)

\chapter{section\label{chapter:IPM}}

The OPF problems can be formulated as a general nonlinear optimal control problem
\begin{subequations}
	\label{eq:NLP}
	\begin{align}
	\min_{\bfx} \qquad & f(\bfx)  \label{eq:NLPobj}\\
	\text{subject to} \qquad &  \bfg(\bfx) = 0,  \label{eq:NLPeq}\\
	&  \bfh(\bfx) \geq 0,  \label{eq:NLPineq}\\
	& \bfx \geq 0, \label{eq:NLPbounds}
	%                       & \underline{\bfx} \leq \bfx \leq \overline{\bfx} \label{eq:NLPbounds},
	\end{align}
\end{subequations}
where $\bfx \in \mathbb{R}^n$ and the objective function $f$ is a mapping $f: \mathbb{R}^n \rightarrow \mathbb{R}$ and the constraints $\bfg: \mathbb{R}^n \rightarrow \mathbb{R}^{n_g}$ and $\bfh: \mathbb{R}^n \rightarrow \mathbb{R}^{n_h}$  are assumed to be sufficiently smooth. Only the lower bounds on $\bfx$ \eqref{eq:NLPbounds} are considered in the following derivations. The equations for the general bounds could be derived accordingly, briefly sketched in the later text. The presented IPM description is based on the \IPOPT{} algorithm \cite{ipoptThesis} and \cite{IPOPT2006}.

The inequality constraints \eqref{eq:NLPineq} can be reformulated as the equality constraints by introducing slack variables $\bfs$ with non-negativity constraint $\bfs \geq \0$. The non-negativity constraints for both $\bfs$ and $\bfx$ are subsequently replaced by standard logarithmic barrier functions, which are added to the objective function with a scaling factor $\mu$.  The resulting barrier sub-problem is
\begin{subequations}
	\label{eq:Barrier}
	\begin{align}
	\min_{\bfx} \qquad & f(\bfx) -  \mu_j \sum_{i=1}^{n} \ln(x_i) - \mu_j \sum_{i=1}^{n_h} \ln(s_i) \label{eq:Barrierobj}\\
	\text{subject to} \qquad &  \bfg(\bfx) = 0,  \label{eq:Barriereq}\\
	&  \bfh(\bfx) - \bfs = 0,  \label{eq:Barrierineq}\\
	& \bfs \geq 0,\  \bfx \geq 0.
	\end{align}
\end{subequations}

The influence of the barrier term is determined by the barrier parameter $\mu_j$ and under certain conditions the solution $\bfx^*$ of the barrier problem \eqref{eq:Barrier} converges to the solution of the original problem \eqref{eq:NLP} as  $\mu \downarrow 0$. Consequently, a strategy to solve the original NLP problem is to solve a sequence of the barrier problems for decreasing parameter $\mu_j$. The solution of each iterate is not relevant for the solution of the original problem, so it can be relaxed only to a certain accuracy and such an approximate solution is used as a starting point for the next iterate of the barrier problem with decreased $\mu_{j+1}$. The strategy for updating the $\mu$ parameter and thus switching to the next barrier sub-problem is discussed in section \ref{sec:Barrier}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Optimality Conditions \label{sec:Optimality}}
The solutions of \eqref{eq:Barrier} are critical points of the Lagrangian function
\begin{align}
    \label{eq:lagrangian}
  L(\bfx, \bfs, \bflambda_g, \bflambda_h) =& f(\bfx) -  \mu_j \sum_{i=1}^{n} \ln(x_i) - \mu_j \sum_{i=1}^{n_h} \ln(s_i)\\
  & - \bflambda_g^{\transpose} \bfg(\bfx) - \bflambda_h^{\transpose} (\bfh(\bfx) - \bfs) \nonumber,
\end{align}
where $\bflambda_g$ and $\bflambda_h$ are the vectors representing the Lagrange multipliers for the equality and inequality SCOPF constraints.
Formulating Karush-Kuhn-Tucker (KKT) conditions directly for the \eqref{eq:lagrangian} would lead to complications, since the barrier terms would introduce $\frac{\mu_j}{x_i}$ which is not defined at a solution $\bfx^*$ of the \eqref{eq:NLP} with an active bound $x^*_i = 0$. Primal-dual interior point methods~\cite{Conn2000, Conn2001} define the dual variables $\bfz$ as
\begin{equation}
z_i = \frac{\mu}{x_i},\ i=1,2,\ldots,n. \label{eq:dualVar}
\end{equation}
The primal-dual equations, equivalent to the perturbed KKT conditions for \eqref{eq:Barrier}, then become
\begin{subequations}
	\label{eq:OC}
	\begin{align}
	\boldsymbol{l}_a := \quad & \nabla_x f(\bfx) - \bfJ^{\transpose}_g \bflambda_g - \bfJ^{\transpose}_h \bflambda_h - \bfz &&= \0, \\
	\boldsymbol{l}_b := \quad & -\mu \boldsymbol{e} - \bfS\bflambda_h &&= \0 \label{eq:OCsecond}, \\
	\boldsymbol{l}_c := \quad & \bfg(\bfx) &&= \0, \\
	\boldsymbol{l}_d := \quad & \bfh(\bfx) - \bfs &&= \0, \\
	\boldsymbol{l}_e :=  \quad& Z\bfx - \mu \boldsymbol{e} &&= \0,  
	\end{align}
\end{subequations}
where the matrix $\boldsymbol{Z} = \text{diag}(\bfz)$. The dual variables $\bfz$ correspond to the multipliers for the bound constraints \eqref{eq:NLPbounds}. Note that \eqref{eq:OCsecond} has been post-multiplied with $\bfS$. Also note that the perturbed KKT conditions for $\mu = 0$, together with $x,z,\lambda \geq 0$ are the KKT condition for the original problem \eqref{eq:NLP}.

%TREATMENT OF THE GENERAL BOX BOUNDS
%The box constraints $\underline{\bfx}$ and $\overline{\bfx}$ on the optimization vector $\bfx$ are approached in a similar manner to the inequality constraints by introducing additional barrier terms $\mu_j \sum_i log(x_i - \underline{x_i})$ and $\mu_j \sum_i log( \overline{x_i} - x_i)$, but in order to avoid cumbersome notation and technical details related to these terms they are omitted from the discussion that follows. 

%The general box constraints for the L <= h(x) <= U require two sets of slack variables, s_min and s_max and addition of the corresponding barrier terms. But since in OPF problems we have only branch flow limits, which represent only the upper bounds h(x) <= U, which can be transformed to  -(h(x) - U) >= 0, which is indeed how it is implemented in IPOPT 
The treatment of the problem with general box constraints $\bfx^{\text{min}} \leq \bfx \leq \bfx^{\text{max}}$ instead of \eqref{eq:NLPbounds} requires the addition of modified logarithmic barrier terms
\begin{equation}
    f_{\mu}(\bfx) = -\mu_j \sum_{i=1}^n \ln(x_i - x_i^{\text{min}}) - \mu_j \sum_{i=1}^n \ln( x_i^{\text{max}} - x_i),
\end{equation}
and the dual variables for $i=1,2,\ldots,n$ become
\begin{align}
z_i^{\text{min}} &= \frac{\mu}{x_i-x_i^{\text{min}}}, \\
z_i^{\text{max}} &= \frac{\mu}{x_i^{\text{max}} - x_i}.
\label{eq:dualVarFULL}
\end{align}
In case there are general bounds for the inequality constraints $\bfh^{\text{min}} \leq \bfh(\bfx) \leq \bfh^{\text{max}}$ instead of \eqref{eq:NLPineq}, the slack variables and Lagrange multipliers need to be introduced for each bound separately. Alternative interpretation of the general bounds can be based on handling the bounds separately, i.e. $\bfh^{\text{min}} \leq \bfh(\bfx)$ and $\bfh(\bfx) \leq \bfh^{\text{max}}$ and introducing new inequality constraints equivalent to the formulation of \eqref{eq:NLPineq}
\begin{equation}
    \bfh'(\bfx) := 
    \begin{bmatrix}
    \bfh(\bfx) - \bfh^{\text{min}}\\
    \bfh^{\text{max}} -\bfh(\bfx)
    \end{bmatrix}
    \geq \0.
\end{equation}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Search Direction Computation  \label{sec:SearchDir}}
Since the solution of the barrier problem \eqref{eq:Barrier} satisfies the perturbed KKT conditions \eqref{eq:OC}, Newton's method may be applied to solve this system of nonlinear equations. The search direction $(\Delta \bfx^k, \Delta \bfs^k, \Delta \bflambda_g^k,\Delta \bflambda_h^k, \Delta \bfz^k)^{\transpose}$ at iteration $k$ can be obtained from the linearization of \eqref{eq:OC} at the iterate $( \bfx^k, \bfs^k, \bflambda_g^k, \bflambda_h^k, \bfz^k)^{\transpose}$, resulting in a system of linear equations
\begin{equation}
\label{eq:SCOPFhessian}
\begin{bmatrix}
\boldsymbol{H} & \0 & -\bfJ^{\transpose}_g & -\bfJ^{\transpose}_h & -\bfI\\
\0 & \bfLambda_h & \0 & \bfS & \0 \\
\bfJ_g & \0 & \0 & \0 & \0\\
\bfJ_h & -\bfI & \0 & \0 & \0\\
\boldsymbol{Z} & \0 & \0 & \0 & \boldsymbol{X}
\end{bmatrix}^k
\begin{bmatrix}
\Delta \bfx^k\\
\Delta \bfs^k\\
\Delta \bflambda_g^k\\
\Delta \bflambda_h^k\\
\Delta \bfz^k\\
\end{bmatrix}
=
-\begin{bmatrix}
\boldsymbol{l}_a \\
\boldsymbol{l}_b \\
\boldsymbol{l}_c \\
\boldsymbol{l}_d \\
\boldsymbol{l}_e
\end{bmatrix}^k,
\end{equation}
%the elimination is performed by multiplying last row with X^-1 and the first with -1, then subtracting the last row from the first
where  $\boldsymbol{H} = \nabla_{xx} L$, and $\bfLambda_h = \text{diag}(\bflambda_h)$. The last block row is eliminated and then the second row of \eref{eq:SCOPFhessian} is post-multiplied with $-\bfS^{-1} $ in order to enforce the symmetry of the KKT system:
\begin{equation}
\label{eq:SCOPFhessianSymmetric}
\begin{bmatrix}
\boldsymbol{\tilde{H}} & \0 & \bfJ^{\transpose}_g & \bfJ^{\transpose}_h \\
\0 & \boldsymbol{L}_{s} & \0 & -\bfI \\
\bfJ_g & \0 & \0 & \0 & \\
\bfJ_h & -\bfI & \0 & \0 & 
\end{bmatrix}^k
\begin{bmatrix}
\Delta \bfx^k\\
\Delta \bfs^k\\
\Delta \bflambda_g^k\\
\Delta \bflambda_h^k
\end{bmatrix}
=
\begin{bmatrix}
\boldsymbol{l}_a + \boldsymbol{X}^{-1} \boldsymbol{l}_e\\
\bfS^{-1} \boldsymbol{l}_b \\
-\boldsymbol{l}_c \\
-\boldsymbol{l}_d
\end{bmatrix}^k,
\end{equation}
where $\boldsymbol{\tilde{H}} = -\boldsymbol{H} - \boldsymbol{X}^{-1}\boldsymbol{Z}$, and the diagonal matrix $\boldsymbol{L}_{s} = -\bfS^{-1}\bfLambda_h$. The eliminated $\Delta \bfz^k$ can be recovered from
\begin{equation}
\label{eq:SCOPFhessianSymmetricRecovery}
    \Delta \bfz^k = -\boldsymbol{X}^{-1} (\boldsymbol{l}_e + \boldsymbol{Z}\Delta \bfx^k).
\end{equation}

In order to obtain robust IPM algorithm it is important to obtain high quality search directions, thus it is crucial to address the accuracy of the LS solution. Most of the burden is shifted to the linear solver, where techniques such as LS fill-in minimization reordering, scaling vectors, matching and pivoting can provide substantial improvement. Additional improvement can be achieved by performing iterative refinement using the unreduced KKT linear system of form \eqref{eq:SCOPFhessian}. 
%%SCHUR SYSTEM SOLUTION TECHNIQUE SEEMS NOT TO PROVIDE ANY IMPROVEMENT USING THE ITERATIVE REFINEMENT, THAT'S WHY COSMIN USED PRECONDITIONED BICGSTAB TO ABSORB THE ERROR

%%%%%%%%%%%%%%%% SLACK ELIMINATION
\subsection{Additional Variables Elimination}
It is possible to further reduce the KKT system by eliminating the slack variables $\bfs$. The system \eqref{eq:SCOPFhessianSymmetric} can be permuted to the structure with the diagonal block $\L_{s}$ in the lower right corner
\begin{equation}
\label{eq:SCOPFslackAtEnd}
\begin{bmatrix}
\tilde{\Hess} & \Jac^{\transpose}_g & \Jac^{\transpose}_h & \0 \\
\Jac_g & \0 & \0 & \0 & \\
\Jac_h & \0 & \0 & -\bfI \\
\0 & \0 & -\bfI & \L_{s}
\end{bmatrix}^k
\begin{bmatrix}
\Delta \bfx^k\\
\Delta \bflambda_g^k\\
\Delta \bflambda_h^k\\
\Delta \bfs^k
\end{bmatrix}
=
\begin{bmatrix}
\boldsymbol{l}_a + \boldsymbol{X}^{-1} \boldsymbol{l}_e\\
-\boldsymbol{l}_c \\
-\boldsymbol{l}_d\\
\Sc^{-1} \boldsymbol{l}_b
\end{bmatrix}^k.
\end{equation}
Given that the block $\L_{s}$ is a diagonal matrix, the reordered system \eqref{eq:SCOPFslackAtEnd} can be further reduced by eliminating the slack variables by performing the Schur complement with respect to the $3 \times 3$ block in the upper left corner,
\begin{equation}
\label{eq:SCOPFhessianSchurComplement}
\begin{bmatrix}
\tilde{\Hess} & \Jac^{\transpose}_g & \Jac^{\transpose}_h \\
\Jac_g & \0 & \0 &  \\
\Jac_h & \0 & \0
\end{bmatrix} -
\begin{bmatrix}
 \0 & \0 & -\bfI
\end{bmatrix}^{\transpose} {(\L_{s})}^{-1}
\begin{bmatrix}
 \0 & \0 & -\bfI
\end{bmatrix}.
\end{equation}
% \begin{equation}
%     A_{11} - A_{12} A_{22}^{-1} A_{21}
% \end{equation}
Forming such Schur complement is trivial since it requires inverting only the diagonal matrix $\L_{s}$.
%The \PARDISO{} LS solver~\cite{pardiso} requires the diagonal entries to be specified in the sparse structure even if they are numerically zero. Considering this fact, the sparse structure of the $3 \times 3$ block Schur complement is not changed since only the diagonal entries are modified.
The reduced linear system that needs to be solved has now the structure
\begin{equation}
\label{eq:SCOPFhessianReduced}
\begin{bmatrix}
\tilde{\Hess} & \Jac^{\transpose}_g & \Jac^{\transpose}_h \\
\Jac_g & \0 & \0 &  \\
\Jac_h & \0 & - \L_{s}^{-1}
\end{bmatrix}
\begin{bmatrix}
\Delta \bfx\\
\Delta \bflambda_g\\
\Delta \bflambda_h\\
\end{bmatrix}
=
\begin{bmatrix}
\boldsymbol{l}_a + \boldsymbol{X}^{-1} \boldsymbol{l}_e\\
-\boldsymbol{l}_c \\
\Sc^{-1} \boldsymbol{l}_b - \L_{s}^{-1} \boldsymbol{l}_d \\
\end{bmatrix}
\end{equation}
and the eliminated slack variables can be recovered by solving
\begin{equation}
\label{eq:SCOPFslackReduction}
\L_{s} \Delta \bfs = \Sc^{-1} \boldsymbol{l}_b + \Delta \bflambda_h.
\end{equation}


\subsection{Inertia Correction and Curvature Detection}
In order to guarantee descent properties for the line-search procedure, it is necessary to ensure that the Hessian matrix projected on the null space of the constraint Jacobian is positive definite. Also, if the constraint Jacobian does not have full rank, the iteration matrix in \eqref{eq:SCOPFhessianSymmetric} is singular, and the solution might not exist. These conditions are satisfied if the iteration matrix has the inertia $(n+n_h,n_g+n_h,0)$, i.e., if it has exactly $n + n_h$ positive, $n_g + n_h$ negative, and no zero eigenvalues. The sizes correspond to the size of the Hessian block (including the slack variables) and the Jacobians of the equality and inequality constraints. If the inertia is not correct, the iteration matrix needs to be modified. In \IPOPT{} implementation, the diagonal perturbation $\delta_w, \delta_c \geq 0$ is added to the Hessian block and the lower right $2 \times 2$ block, respectively. The system is re-factorized with different trial values of $\delta_w, \delta_c$ until the inertia is correct. The inertia of the iteration matrix is readily available from several sparse indefinite linear solvers, such as \PARDISO{} \cite{SCHENK2001}. In case the correct inertia cannot be achieved, the current search direction computation is aborted and the algorithm uses different objective function that does try to solely minimize the feasibility violation (e.g. minimizing the constraints violation), ignoring the original objective function, hoping that the matrix has better properties close to the feasible points.

The inertia detection strategy focuses on the properties of the augmented iteration matrix \eqref{eq:SCOPFhessianSymmetric} alone and can thus discard search directions that are of descent but for which the inertia of the augmented matrix is not correct. Furthermore, the inertia detection strategy might require multiple re-factorization of the iteration matrix and, because the factorization is the most expensive step in the algorithm, computational performance can be greatly affected. Furthermore, the inertia estimates might vary, depending on used linear solver or not be available at all. To bypass the need for inertia information, several authors suggest to use the curvature test \eqref{eq:curvature}, e.g. \cite{Chiang2016}, \cite{CosminCurvature}.
\begin{align}
\label{eq:curvature}
& \bfd_k^{\transpose} \boldsymbol{W}_k(\delta) \bfd_k \geq \kappa \bfd_k^{\transpose} \bfd_k, \quad \kappa > 0, \\
\nonumber
& \boldsymbol{W}_k(\delta) = 
 \begin{bmatrix}
 \boldsymbol{\tilde{H}} & \0 \\
 \0 & \boldsymbol{L}_{s}
 \end{bmatrix}^k + \delta \bfI, \quad \bfd_k = [\Delta \bfx^{\transpose}_k, \Delta \bfs^{\transpose}_k]^{\transpose}.
\end{align}
If the test is satisfied, the search direction is accepted; if not satisfied, the regularization parameter $\delta$ is increased and new search direction is computed using the new regularized matrix. While the curvature detection strategy requires more iterations compared with inertia detection, it also requires less extra factorizations. Thus the solution time is less than that of inertia detection because significantly fewer regularizations are needed. In a parallel computing context this result is relevant because curvature detection reduces the number of times that the system needs to be assembled and solved, which is the parallelization bottleneck.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Backtracking Line-search Filter Method  \label{sec:FilterLS}}
After the successful computation of the search direction from \eqref{eq:SCOPFhessianSymmetric} and \eqref{eq:SCOPFhessianSymmetricRecovery} the step sizes $\alpha_k, \alpha_k^z \in (0,1]$ need to be determined in order to obtain the next iterate 
\begin{align}
\bfx^{k+1} &= \bfx^{k} + \alpha_k \Delta \bfx^k,\\
\bfs^{k+1} &= \bfs^{k} + \alpha_k \Delta \bfs^k,\\
\bflambda_g^{k+1} &= \bflambda_g^{k} + \alpha_k^z \Delta \bflambda_g^k,\\
\bflambda_h^{k+1} &= \bflambda_h^{k} + \alpha_k^z \Delta \bflambda_h^k,\\
\bfz^{k+1} &= \bfz^{k} + \alpha_k^z \Delta \bfz^k.
\end{align}
%NOTE: in the IPOPT implementation paper alpha_z is used only for z (nod lambdas), but in the step A-6 of algorithm A it is used also for the lambdas, which makes more sense.
Different step in the dual variables is allowed in order not to unnecessary restrict the other variables. A first candidate step length is chosen such that the strict positivity of $\bfx, \bfs$ and $\bfz$ is preserved, since it needs to hold both in the solution of the barrier problem \eqref{eq:Barrier} and also in every iteration, which is necessary in order to evaluate the barrier function. This is accomplished by fraction-to-the-boundary rule, which identifies the maximum step size $\alpha_k, \alpha^z_k \in (0,1]$ such that
\begin{align}
    \alpha^{max}_k &= \max \left(\alpha \in (0,1]: \bfx^{k} + \alpha \Delta \bfx^k \geq (1-\tau)\bfx^k \right),\\
    \alpha_k^z &= \max \left(\alpha \in (0,1]: \bfz^{k} + \alpha \Delta \bfz^k \geq (1-\tau)\bfz^k \right),
\end{align}
where $\tau \in (0,1)$ is a function of the current barrier parameter $\mu_j$.  The step size for the dual variables $\alpha^z_k$ is used directly, but in order to ensure global convergence the step size $\alpha_k \in (0,\alpha_k^{max})$ for the remaining variables is determined by a backtracking line-search procedure, exploring a decreasing sequence of trial step sizes $\alpha_k^i = 2^{-i} \alpha_k^{max}$ for $i = 0,1,2,\ldots$.

The variant of backtracking line-search filter method \cite{Fletcher2002} used in \IPOPT{} is based on the idea of bi-objective optimization problem with the two goals, (i) minimizing the objective function 
\begin{equation}
\varphi_{\mu_j}(\bfx,\bfs) := f(\bfx) -  \mu_j \sum_{i=1}^{n} \ln(x_i) - \mu_j \sum_{i=1}^{n_h} \ln(s_i),
\end{equation}
and (ii) minimizing the constraint violation
\begin{equation}
\theta(\bfx,\bfs) := ||\  [\bfg(\bfx)^{\transpose} \ \ (\bfh(\bfx)-\bfs)^{\transpose}]^{\transpose} \  ||_1.    
\end{equation}
A trial point
$\bfx^{k}(\alpha_k^i) := \bfx^{k} + \alpha_k^i \Delta \bfx^k$ and 
$\bfs^{k}(\alpha_k^i) := \bfs^{k} + \alpha_k^i \Delta \bfs^k$
during the backtracking line search is considered to be acceptable, if it leads to sufficient progress toward either goal compared to the current iterate. The emphasis is put on the latter goal, until the constraint violations satisfy a certain threshold. Afterwards, the former goal is emphasized and reduction in the barrier function is required, accepting only iterates satisfying Armijo condition.% \cite{NocedalBookOptim}.

The algorithm also maintains a filter, defined as a set 
\begin{equation}
    \mathcal{F}_j \subseteq \{(\theta, \varphi) \in \mathbb{R}^2 : \theta >0 \},
\end{equation}
for each barrier sub-problem $j$ for which the $\mu_j$ is fixed. The filter $\mathcal{F}_j$ contains those combinations of constraint violation values $\theta$ and the objective function values $\varphi$, that are prohibited for a successful trial point in all iterations within the $j$-th barrier sub-problem. The filter is initialized so that the algorithm will never allow trial points to be accepted that have a constraint violation larger than $\theta^{max}$. During the line search, a trial point $\bfx^k(\alpha_k^i),\ \bfs^{k}(\alpha_k^i)$ is rejected, if $(\theta(\bfx_k(\alpha_k^i), \bfs^{k}(\alpha_k^i)),\ \varphi_{\mu_j}(\bfx^k(\alpha_k^i), \bfs^{k}(\alpha_k^i))) \in \mathcal{F}_j$. After every iteration, in which the accepted trial step size does not satisfy the two objectives of the backtracking line-search, the filter is augmented. This ensures that the iterates cannot return to the neighborhood of the unsatisfactory iterates. Overall, this procedure ensures that the algorithm cannot cycle, for example between two points that alternate between decrease of the constraint violation and the barrier objective function.

In cases when it is not possible to identify a satisfactory trial step size, the algorithm reverts to a feasibility restoration phase. Here, the algorithm tries to find a new iterate which is acceptable to the current filter, by reducing the constraint violation with some iterative method. Note that the restoration phase algorithm might not be able to produce a new iterate for the filter line-search method, for example, when the problem is infeasible.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Barrier Parameter Update Strategy  \label{sec:Barrier}}
The strategy of the barrier parameter update is an important factor influencing the convergence properties, especially for difficult nonconvex problems such as OPF. When solving nonlinear nonconvex programming problems, much caution must be exercised to prevent the iteration from failing. Non-minimizing stationary points can attract the iteration, and aggressive decreases in the barrier parameter can lead to failure. 
%A smooth, gradual decrease of the barrier parameter keeps the IPM trajectory close to the central path. On the other hand, more rapid change in the barrier parameter leads to more erratic steps in the Newton direction. [https://www.youtube.com/watch?v=MsgpSl5JRbI]
Different barrier parameter update strategies are discussed here, including the monotone Fiacco-McCormick strategy \cite{muMONOTONE} and an adaptive strategy based on minimization of a quality function \cite{muADAPTIVEqualityfcn}.

\subsubsection{Monotone Strategy}
Using the default monotone Fiacco-McCormick strategy, an approximate solution to the barrier problem \eqref{eq:Barrier} for a fixed value of $\mu$ is computed, possibly iterating over multiple primal-dual steps. Subsequently, the barrier parameter is updated and the computation continues by solution of the next barrier problem, starting from the approximate solution of the previous one. The approximate solution for the barrier problem \eqref{eq:Barrier}, for a given value of $\mu_j$, is required to satisfy the tolerance
\begin{equation}
    E_{\mu}(\bfx^{j+1}, \bfs^{j+1}, \bflambda_g^{j+1}, \bflambda_h^{j+1}, \bfz^{j+1}) <  \kappa_{\epsilon} \mu_j
\end{equation}
for a constant $\kappa_{\epsilon}>0$ before the algorithm continues with the solution of the next barrier problem. The optimality error for the barrier problem is defined by considering the individual parts of the primal-dual equations \eqref{eq:OC}, that is the dual feasibility (optimality), primal feasibility (constraint violations), and the complementarity conditions,
\begin{equation}
\label{eq:NLPerror}
  E_{\mu}(\bfx, \bfs, \bflambda_g, \bflambda_h, \bfz) = 
  \max \left(
    ||\boldsymbol{l}_a||_{\infty},
    ||\boldsymbol{l}_b||_{\infty},
    ||\boldsymbol{l}_c||_{\infty},
    ||\boldsymbol{l}_d||_{\infty},
    ||\boldsymbol{l}_e||_{\infty}
  \right).
\end{equation} 

In the monotone barrier update strategy, the new barrier parameter is obtained from
\begin{equation}
\label{eq:MUupdate}
    \mu_{j+1} = \max \left( \frac{\epsilon_{tol}}{10},\  \min \left(\kappa_{\mu} \mu_j,\  \mu_j^{\theta_{\mu}} \right) \right),
\end{equation}
with constants $\kappa_{\mu} \in (0,1)$ and $\theta_{\mu} \in (1,2)$. In this way, the barrier parameter is eventually decreased at a superlinear rate. On the other hand, the update rule \eqref{eq:MUupdate} does not allow $\mu$ to become smaller than necessary given the desired tolerance $\epsilon_{tol}$, thus avoiding numerical difficulties at the end of the optimization procedure.

The monotone Fiacco-McCormick strategy can be very sensitive to the choice of the initial point, the initial value of the barrier parameter and the scaling of the problem. Furthermore, different problems might favour strategies for selecting the barrier parameter at every iteration of an interior-point method, that is for every primal-dual step computation. Two adaptive strategies implemented in \IPOPT{} are discussed next.

\subsubsection{Adaptive Strategies}
%The paper in \cite{muADAPTIVEqualityfcn} discusses the problem with equality constraints only, but in the discussion here we have inequality constraints as well. What it means is that their x is our [x s] and their z is our z as well (since we do not introduce the dual variables for slacks because S^-1 was eliminated by post-multiplication by S, therefore we don't have any 1/s_i terms). What does this mean for our discussion? How is the complementarity gap computed? is their x the same as our x (excluding s)?
The most common approach for choosing the barrier parameter $\mu$ in the adaptive methods is to make it proportional to the complementarity value in the current iterate
\begin{equation}
    \mu = \sigma \frac{\bfx^{\transpose} \bfz}{n},
\end{equation}
where $\sigma > 0$ is a centering parameter and $n$ denotes the number of primal variables. The adaptive strategies vary in how the centering parameter is determined. 

In Mehrotra's probing heuristic \cite{muADAPTIVEmehrotra}, which uses the predictor-corrector principle to compute the search direction, the $\sigma$ is computed as the ratio between the complementarity value in the current iterate and the iterate updated by the predictor step, considering the longest possible step sizes that retain the non-negativity of the variables in the barrier problem. If good progress in the complementarity value is made in the predictor step, the centering parameter obtained in this way is small, $\sigma < 1$, therefore the $\mu$ will be small in the next iteration. In other cases $\sigma$ may be chosen to be greater than $1$. This heuristic is based on experimentation with linear programming problems, and has proved to be effective for convex quadratic programming as well.

The adaptive barrier update strategy based on quality function, as suggested in \cite{muADAPTIVEqualityfcn}, is trying to determine the $\sigma$ value to be such that it minimizes the linear approximation of the quality function. The quality function is a measure defined by the infeasibility norms in the current iterate updated by the probing search direction, which is expressed as a function of the sought $\sigma$. The minimization problem is solved by golden bisection procedure on the specified $(\sigma_{min}, \sigma_{max})$ interval with maximum of 12 bisections.

%{\color{red}TODO: Is this description enough? Should I introduce also the formal definitions and all the theory (requires 1 page each)}

The evaluation of the barrier update strategies on both linear and nonlinear problems revealed superior performance of the adaptive methods over the monotone strategy, both in terms of CPU time and number of IPM iterations. Although the results were more pronounced on the linear benchmarks, significant improvements can be expected by using adaptive strategies, particularly in applications where the function evaluation has the dominant cost \cite{muADAPTIVEqualityfcn}.
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Problem Scaling and Convergence Criteria  \label{sec:Scaling}}
%scaling of the variables and gradients [http://www.alglib.net/optimization/tipsandtricks.php]
Real-life optimization problems often have parameters with different magnitudes. Such badly scaled  problems are hard to solve because of two reasons. First, different magnitude of the variables makes it hard to formulate reasonable stopping criteria. For example, sufficiently small step in one variable might not be enough for another variable which is many orders of magnitude smaller. Second, different magnitude of variables increases condition number of the associated LS - hence the search direction might not be accurate enough and the optimizer needs more iterations to converge. In the OPF context, the voltage variables are usually well scaled, since we consider voltage magnitudes in per unit scale (relative to the voltage setpoint) and voltage angles are given in radians. The generator power output is similarly converted to per unit quantities.
%TODO: experiment with scaling of the OPF variables so that their magnitude is ~1 (e.g. dump the x_0 to see what is the rage of values there, is it close to 1?? what are the actual orders of the Va,Vm,Pg,Qg??)
%RESULTS
%VA,VM are fine, in the same order of magnitude
%PG, QG may vary, the bounds min max are spanning 3 order of magnitude
%%Problem: the big differences occur as some variables approach the bound 0 (1e-8 or so), which causes orders of magnitude difference => although in practice the output 1e-2 or 1e-8 is probably the same (how many digits of precision are assumed??), we consider such values to be zero
%TODO: exmeriment with IPM iterations using different scaling, use case13659pegase_fixed, it is nicely visible there, even does not converge

In ideal case, not only the variables but also the functions should be scaled so that changing a variable by a given amount has a comparable effect on any function which depends on this variables, or in other words, so that the non-zero elements of the function gradients are of the same order of magnitude. For this purpose, also the gradient scaling needs to be addressed. The scaling factors for the gradients are defined as
\begin{align}
    s_f   &= \min (1,\ g_{max} / ||\nabla_x f(\bfx_0)||_{\infty}), \\
    s_g^{(j)} &= \min (1,\ g_{max} / ||\nabla_x g^{(j)}(\bfx_0)||_{\infty}),\  j=1\ldots n_g \\
    s_h^{(j)} &= \min (1,\ g_{max} / ||\nabla_x h^{(j)}(\bfx_0)||_{\infty}),\ j=1\ldots n_h.
\end{align}
for a given $g_{max} > 0$. If the maximum gradient is above this value, then gradient based scaling will be performed. Note that all gradient components in the scaled problem are at most of the size $g_{max}$ at the starting point. The scaling factors are computed only at the beginning of the optimization using the starting point and kept constant throughout the whole optimization process.

Even if the original problem is well scaled, the multipliers $\bflambda_g, \bflambda_h, \bfz$ might become very large, for example, when the gradients of the active constraints are (nearly) linearly dependent at a solution of \eqref{eq:NLP}. In this case, the algorithm might encounter numerical difficulties satisfying the unscaled primal-dual equations \eqref{eq:SCOPFhessianSymmetric} to a tight tolerance. The convergence criteria in \eqref{eq:NLPerror} therefore need to be scaled accordingly. The scaled optimality error used to determine the convergence criteria is defined as
\begin{equation}
\label{eq:NLPerrorScaled}
  E_0(\bfx, \bfs, \bflambda_g, \bflambda_h, \bfz) = 
  \max \left(
    \frac{||\boldsymbol{l}_a||_{\infty}}{s_1},
    \frac{||\boldsymbol{l}_b||_{\infty}}{s_1},
    ||\boldsymbol{l}_c||_{\infty},
    ||\boldsymbol{l}_d||_{\infty},
    \frac{||\boldsymbol{l}_e||_{\infty}}{s_2}
  \right),
\end{equation}
where the scaling factors $s_1, s_2$ are defined as
\begin{equation}
    s_1 = \dfrac{\max \left( s_{max}, \frac{||\bflambda_g||_1 + ||\bflambda_h||_1 + ||\bfz||_1}{n_g + n_h + n} \right)}{s_{max}}, \quad s_2 = \dfrac{\max \left( s_{max}, \frac{||\bfz||_1}{n} \right)}{s_{max}}.
\end{equation}

The overall \IPOPT{} algorithm terminates successfully, if the NLP error for the current iterate for $\mu = 0$ in \eqref{eq:NLPerrorScaled},
\begin{equation}
  \label{eq:NLPerrorZERO}
  E_{0}(\bfx, \bfs, \bflambda_g, \bflambda_h, \bfz) \leq \epsilon_{tol},
\end{equation}
becomes smaller than the user provided value $\epsilon_{tol} >0$, and if the individual criteria according to dual, primal, and complementarity conditions in \eqref{eq:NLPerrorScaled} are met. Each criterion uses separate, user provided tolerance value.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Overall primal-dual IPM algorithm  \label{sec:IPMalgorithm}}
%TODO

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Initial Point Selection and Warm-start Strategies  \label{sec:Warmstart}}
%TODO: how is x, z_l, z_u and z selected (ad implementation paper)
%also the OPF context selection of x

The simplex method moves from vertex to vertex of the polytope encompassing the feasible set. In the typical case, a reasonably small change in the objective will result in a new optimal solution that is only a few simplex pivots away. An optimal basis of an original problem usually serves as an excellent warm-start to resolve another closely related problem.

Unlike  the  simplex  method,  IPMs  generate  a  sequence of interior-points that converge to an optimal solution in the limit. Since IPMs work with interior-points, they tend to generate much better search directions at points that are away from the boundary of the feasible region and close to the central path. When the new optimization problem is being solved, using and optimal solution of a near problem, it might take several iterations just to get back to the central path. Therefore, an optimal or a near-optimal solution of the original problem is in general not a very good candidate to be used as a warm-start for the solution of a nearby problem. Approaches proposed in the existing literature on warm-start strategies and reoptimization in the context of IPMs relies on the set of starting points with desirable properties such as near-feasibility, near-optimality, and/or proximity to the central path \cite{IPMwarm}.

Typically, after perturbing the original problem, the previous solution fails to satisfy primal feasibility or dual feasibility or both. The existing methods propose different ways to handle this situation. Some strategies rely on computing an adjustment or several adjustments to the previously stored iterate to regain feasibility for the perturbed problem, which might reduce the number of iterations, but introduces additional computational cost required to compute the adjustments for the initial guess. Other methods modify the perturbed problem using judiciously chosen penalty or barrier parameters so that the stored iterate can be used as is. This however requires user experience in order to properly determine the appropriate barrier parameter values.
% judiciously chosen penalty or barrier parameters so that the stored iterate can be used as is (show the experimental data - /Users/Juraj/Dropbox/USI/PhD/reports/SCOPF/iters\_x0)

In context of the OPF problems, the warm start strategy considered is that the solution of the original OPF problem is known (both primal and dual variables) and it is used as an initial guess for a nearby problems with perturbed parameters, or with additional variables and constraints.

\subsubsection{Constant Problem Dimension}
In constant problem dimension case the problem size is fixed, i.e. the number of variables and constraints for a nearby problem is not changed with respect to the original problem. Instead, the parameters of the original problems are perturbed, thus obtaining the instance of a nearby problem. This situation arises in situations where system operators need to recompute the OPF problem with updated power demand (or other updated problem parameters), while keeping the rest of the problem unchanged.

%%TODO - changing the demand, which is not part of the control (done, below)
%%TODO - changing the state parameters - e.g. bounds for the lines
%%TODO - changing the control parameters, e.g. the bounds for generators

%%TODO: this should go to the numerical experiments description/results
Warm-start for perturbed demand (tested up to 10\% perturbation) works well, resulting into fewer iterations than the cold start. Initializing also the constraint multipliers with the OPF optimal values results into fewer iterations (as opposed to initializing only the primal variables $x$). Smaller value of the barrier parameters results into better performance, since the constraints are close to feasibility.

%%TODO - using an approximate solution to warms start the IPM
% Using perturbed $x_0$ greatly degrades the IPM iterations count, resulting into more iterations than the cold start (trying to perturb only x, using default/optimal/perturbed lambda).
% Initializing $\mu$ by computing its optimal value as average of $\mu = z_L (x-x_{min})$ and $\mu = z_U (x_{max} - x)$ does not produce minimal number of iterations, other $\mu$ values are more appropriate. Making corrections for the violated bounds after the perturbation of the x also doesn't help.

\subsubsection{Additional Variables and Constraints}
In the second case, the warm start strategies for the nearby problem obtained by adding variables and constraints to the original problem is explored. Such situation arises, e.g. in case of the SCOPF problem, where additional constraints, and thus additional state variables, are added to the original problem.

%TODO:Results, write better
Warm-start in the SCOPF slightly improves the iteration count when initializing only the primal variables $x$. Initializing also the Lagrange multipliers is very likely to exceed the iterations count of the cold start. The choice of the barrier parameter should reflect number of added constraints, the more are added, the larger it should be.

==> 02PowerGrid.tex <==
\chapter{Power Grid}
Merge materials from the OPF (formulations) and SCOPF paper (the grid model).

==> 03parallelKKT.tex <==
\section{Parallel Linear Algebra Components \label{chapter:parallelKKT}}

Computers have evolved significantly over the past decade, at an even faster pace than the power grid. Multicore and many-core computer architectures and distributed compute clusters are ubiquitous today, while the easy performance gains when sequential computing applications simply got faster due to the increased performance and clock frequencies of newer processors, are gone. Performance gains can result only from algorithmic redesign, tailored to the particular application from the ground up, and which is also able to utilize the available hardware of multi- and many-core architectures with deep memory hierarchies. More importantly, the practical efficiency of the IPM algorithms is highly dependant on the linear algebra kernels used.
%Performance gains must be realized through the use of sophisticated algorithms utilizing parallelism across all cores of processors or distributed memory clusters. 
For large-scale SCOPF problems, the computation of the search direction determines the overall run time. Hence, any attempt at accelerating the solution should be focused on the efficient solution of the KKT linear system.

%\section{Parallel Solution of the KKT System \label{sec:schur}}
A widespread approach for solving KKT systems consists of employing black-box techniques of direct sparse solvers, due to their accuracy and robustness. However, these solvers are not aware of the underlying structural properties of the KKT systems arising from the SCOPF problem which makes it possible to significantly decrease time to solution by employing structure exploiting algorithms and parallel computing. The appropriate structure emerges from the fact that each of the variables in the optimization vector
%$[ \bfx^{\transpose}, \s^{\transpose}, \bflambda_g^{\transpose}, \bflambda_h^{\transpose}]^{\transpose}$ %%%%WITH SLACK
$[ \bfx^{\transpose}, \bflambda_g^{\transpose}, \bflambda_h^{\transpose}]^{\transpose}$ %%%%WITHOUT SLACK
corresponds to some contingency scenario $c \in \{0,1,\ldots, N_c\}$,
%where the ordering of the $\bfx$ is defined in \eqref{eq:SCOPFx}. Similar ordering applies to the Lagrange multipliers for the equality and inequality constraints,
%%WITH or WITHOUT SLACK
\begin{align}
	\bfx &= [\bfx_0^{\transpose},\ \bfx_1^{\transpose}, \ldots,\ \bfx_{N_c}^{\transpose},\ \bfx_g^{\transpose}]^{\transpose}, \\ %\s &= [\s_0^{\transpose},\ \s_1^{\transpose}, \ldots,\ \s_{N_c}^{\transpose}]^{\transpose}, \\
	\bflambda_g &= [{\bflambda_g}_0^{\transpose},\ {\bflambda_g}_1^{\transpose}, \ldots,\ {\bflambda_g}_{N_c}^{\transpose}]^{\transpose}, \\
	\bflambda_h &= [{\bflambda_h}_0^{\transpose},\ {\bflambda_h}_1^{\transpose}, \ldots,\ {\bflambda_h}_{N_c}^{\transpose}]^{\transpose} .
\end{align}
In order to reveal the scenario-local structure of the KKT system, the variables corresponding to the same contingency are grouped together, i.e.,
\begin{equation}
	%\bfu_n = [\bfx_n^{\transpose},\ \bflambda_g_n^{\transpose},\ \bflambda_h_n^{\transpose},\s_n^{\transpose}]^{\transpose} %%%WITH SLACK
	\bfu_n = [\bfx^{\transpose},\ \bflambda_g^{\transpose},\ \bflambda_h^{\transpose}]^{\transpose}_n %%%%WITHOUT SLACK
\end{equation}
for $n=0,1,\ldots,N_c$ and thus the global ordering will be
\begin{equation}
\bfu = [\bfu_0^{\transpose},\ \bfu_1^{\transpose}, \ldots,\ \bfu_n^{\transpose},\ \bfu_g^{\transpose}]^{\transpose}, \label{eq:ordering}
\end{equation}
where the variables $\bfu_g = \bfx_g$ are placed at the end of the new optimization vector $\bfu$. These variables couple all the scenarios together by introducing linear relationships between variables corresponding to individual scenarios. Under the new ordering \eqref{eq:ordering}, the KKT system obtains the primal-dual angular structure
\begin{equation}
\label{eq:hessianPerm}
\begin{pmatrix}
	A_0 &        &            &                & B_0^{\transpose} \\
		   & A_1 &	           &                & B_1^{\transpose} \\
		   &        & \ddots &                & \vdots \\
		   & 	    &            &   A_{n}     & B_{n}^{\transpose}\\
	B_0  & B_1 &   \ldots &   B_{n}   &   C
\end{pmatrix}
\begin{pmatrix}
	\Delta \bfu_0\\
	\Delta \bfu_1 \\
	\vdots\\
	\Delta \bfu_n\\
	\Delta \bfu_g
\end{pmatrix} = 
\begin{pmatrix}
	\b_0\\
	\b_1 \\
	\vdots\\
	\b_n\\
	\b_C
\end{pmatrix}.
\end{equation}
% where
% %%WITH SLACK
% % \begin{equation}
% % 	A_i = \begin{pmatrix}
% % 	\Hess_i & \Jac_{g_i}^{\transpose} & \Jac_{h_i}^{\transpose} & \0  \\
% % 	\Jac_{g_i} & \0 & \0  & \0  \\
% % 	\Jac_{h_i} & \0  & \0  & -\IdentityBF \\
% % 	\0  & \0  & -\IdentityBF & \L_{s_i}
% % 	\end{pmatrix}
% % \end{equation}
% %%WITHOUT SLACK
% \begin{equation}
% 	A_i = \begin{pmatrix}
% 	\Hess_i & \Jac_{g_i}^{\transpose} & \Jac_{h_i}^{\transpose}  \\
% 	\Jac_{g_i} & \0 & \0 \\
% 	\Jac_{h_i} & \0  & -\L_{s_i}^{-1}
% 	\end{pmatrix}
% \end{equation}
% contains blocks of the reordered KKT system corresponding to the Hessian with respect to the local variables $\bfu_i$ of the scenario $i$, while block $C$ contains a Hessian with respect to the global variables $\bfu_g$. Hessians with respect to a combination of local and global variables are contained in  blocks $B_i$.

\section{Schur Complement}
% The systems with primal-dual angular form, such as \eqref{eq:hessianPerm}, are well suited to be solved by the Schur complement technique. The Schur complement arises as the result of performing a block Gaussian elimination, thus reducing the problem from the full KKT system into smaller problems corresponding to the diagonal blocks $A_i$ and the dense Schur complement system $S$. 

The direct factorization of the full KKT system is not feasible for large-scale SCOPF problems due to its size and associated factorization fill-in, which would quickly exhaust available memory. Instead, the solution is obtained by a sequence of partial steps, summarized in Algorithm \ref{alg:Schur}. First, the Schur complement $S$ is formed
\begin{equation}
	S = C - \sum_{i=0}^{n} B_i A_i^{-1} B_i^{\transpose}, \label{eq:SCform}
\end{equation}
which, in the general case, becomes a dense matrix. Because the size of the coupling stays constant, independent of the number of contingency scenarios, the size of the $S$ does not increase with an increasing number of contingencies. It can be solved using the dense $LDL^{\transpose}$ factorization and back substitution algorithms. The solution of the dense Schur system
\begin{equation}
	S \Delta \bfu_g =  \b_C - \sum_{i=0}^{n_p} B_i A_i^{-1} \b_i, \label{eq:SCsolve}
\end{equation}
yields a part of the solution corresponding to the coupling variables $\Delta \bfu_g$, which is used to obtain all the local solutions $\Delta \bfu_i$ by solving 
\begin{equation}
	A_i \Delta \bfu_i = \b_i - B_i ^{\transpose}\Delta \bfu_g . \label{eq:SCsolve1}
\end{equation}
This approach allows for a great degree of parallelism. The local Schur complement contributions $B_i A_i^{-1} B_i^{\transpose}$ can be evaluated in parallel, as well as the residuals $B_i A_i^{-1} \b_i$ and the solution $\Delta \bfu_i$ can be computed independently at each process. Interprocess communication occurs as the local Schur complement contributions and residuals need to be reduced to a single process and later during the broadcast of the solution $\bfu_g$ to the rest of the processes. The sequential steps of the Algorithm  \ref{alg:Schur} are indicated as \textit{master}. The collective communication routines, such as reduction and broadcast, are also denoted using the same label; in this case it specifies the root process of collective communication, i.e., \textit{master} will contain the result after the reduction or \textit{master}'s data are broadcasted to other processes.

%\subsection{Multicore Sparse Linear Algebra} \label{sec:augmented}
\section{Multicore Local Schur Complement} \label{sec:augmented}
The most expensive step of the presented computational scheme is evaluation of the local contributions to the Schur complement $B_i A_i^{-1} B_i^{\transpose}$ in \eqref{eq:SCform}. The standard approach uses a direct sparse solver such as \PARDISO{}~\cite{SCHENK2001}, to factorize the symmetric matrix $A_i = L_iD_iL_i^{\transpose}$ and perform multiple forward-backward substitutions with all right-hand side (RHS) vectors in $B_i^{\transpose}$, followed by multiplication from the left by $B_i$. This approach, however, does not exploit sparsity of the problem in $B_i^{\transpose}$ blocks, since the linear solver treats the RHS vectors as being dense. 
%Furthermore, the triangular solves with $L_i, L_i^{\transpose}$ do not scale well with the number of cores in multicore environments, since they are memory bound.

An alternative approach, implemented in \PARDISO{}, addresses these limitations by performing an incomplete factorization of the augmented matrix $M_i$~\cite{olafAugmented} exploiting also the sparsity of $B_i^{\transpose}$. The factorization of the augmented matrix $M_i$,
\begin{equation}
	M_i = \begin{pmatrix}
	A_i & B_i^{\transpose} \\
	B_i & 0
	\end{pmatrix},
	\label{eq:augmented} 
\end{equation}
is stopped after pivoting reaches the last diagonal entry of $A_i$. At this point, the term $-B_i A_i^{-1} B_i^{\transpose}$ is computed and resides in the (2, 2) block of $M_i$. By exploiting the sparsity not only in $A_i$, but also in $B_i$ it is possible to reduce memory traffic by using in-memory sparse matrix compression techniques, which render this approach quite favorable for multicore parallelization.
\begin{algorithm}[t]
	\caption{ Parallel procedure for solving the linear systems with the block diagonal arrowhead structure \eqref{eq:hessianPerm} based on the Schur complement decomposition \eqref{eq:SCform}--\eqref{eq:SCsolve1}.}
	Distribute blocks from the KKT system evenly across $\mathcal{P}$ processes, where $\mathcal{N}_p$ is the set of blocks assigned to process $p \in \mathcal{P}$. Each process executes the following procedure:
	\begin{algorithmic}[1]
		\Procedure{SchurSolve}{KKT, $\Delta \bfu$ ,$\b$}
			\State Factorize $A_i = L_i D_i L_i^{\transpose}$ for each $i \in \mathcal{N}_p$\label{alg:SchurSCf1} 
			\State Compute $S_i = B_i A_i^{-1} B_i^{\transpose}$ for each $i \in \mathcal{N}_p$
			\State Accumulate $C_p = \sum_{i \in \mathcal{N}_p} S_i$
			\State Reduce $S = C - \sum_{p \in \mathcal{P}} C_p$ \Comment{master}\label{alg:SchurSCf2} 
			\State Factorize $S = L_s D_s L_s^{\transpose}$ \Comment{master}\label{alg:schurF}
			\State Compute $r_i =  B_i A_i^{-1} b_i$ for each $i \in \mathcal{N}_p$ \label{alg:SchurRHS}
			\State Accumulate $r_p =  \sum_{p \in \mathcal{P}} r_i$ 
			\State Reduce $r =  \sum_{p \in \mathcal{P}} r_p$ \Comment{master}
			\State Solve $S \Delta \bfu_g =  \b_C - r$ \Comment{master}\label{alg:schurS}
			\State Broadcast solution $\bfu_g$ to all $p \in \mathcal{P}$ \Comment{master}\label{alg:solve1}
			\State Solve $A_i \Delta \bfu_i = B_i \bfu_g - \b_i $  for each $i \in \mathcal{N}_p$ \label{alg:solve2}
			\EndProcedure
	\end{algorithmic}
	\label{alg:Schur}
\end{algorithm}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\section{Numerical Results}
% In this chapter we first describe the hardware and software setup used in the experiments and  demonstrate the impact of the KKT system solution phase on the overall computational time of IPM algorithm. We demonstrate that the direct solution approach and the distributed solution approach based on the Schur complement decomposition lead to the same SCOPF solution and we report on benefits of the improved sparse linear algebra and slack variables elimination in computation of the local Schur complement contributions. 
%The small problem sizes are chosen for these tests in order to obtain serial solutions in reasonable time.

Time-to-solution and scaling of the parallel and distributed memory solution is reported for multiple large-scale SCOPF problems. Furthermore, the bottlenecks of the decomposition scheme and their impact on the performance are discussed. 
%Second, preliminary study of the reduced space approach is performed.
 
In what follows, a direct sparse solution of the KKT will be referred to as ``Direct'', while the parallel solution approach based on the Schur complement decomposition is referred to as '\mbox{\BELTISTOS{}-N}', where N denotes the number of parallel processes. 
We further distinguish between standard ``backsolve" approach to local Schur complement computation, indicated by '\BELTISTOS{}-N-std', while the approach where the local Schur complement contributions are obtained by factorization of the augmented matrix \eqref{eq:augmented} is denoted as '\BELTISTOS{}-N-aug'. Multicore augmented factorization approach with T threads is further denoted as '\BELTISTOS{}-N-aug-T'. The notation is summarized in Table~\ref{tab:naming}.
%\cite{DrososMPOPF}

\pgfplotstableread{
Method    Description
{Direct} {Direct sparse solver (\PARDISO{}).}
{\BELTISTOS{}-N-std} {Algorithm~\ref{alg:Schur} using N processes.}
{\BELTISTOS{}-N-aug} {Algorithm~\ref{alg:Schur} with \eqref{eq:augmented} using N processes.}
{\BELTISTOS{}-N-aug-T} {Multicore execution with T threads.}
}\methods

\begin{table}[!ht]
    \footnotesize
	\centering
	\caption{Summary of the notation. \label{tab:naming}}
	\pgfplotstabletypeset[
	every head row/.style={ before row={\toprule},after row=\midrule},
	every last row/.style={ after row=\bottomrule},
%	precision=2, fixed zerofill, column type={r},
%	columns/Statistic/.style={string type,column type=l},
% 	every row/.style={
% 		column type=r,
% 		dec sep align,
% 		fixed,
% 		fixed zerofill,
% 	},
	every odd row/.style={before row={\rowcolor{tablecolor1}}},
    every even row/.style={before row={\rowcolor{tablecolor2}}},
	every column/.style={string type, column type={l}},
	columns/{N=120}/.style={column name={$N=120$}},
	empty cells with={---} % replace empty cells with ’--’
	]\methods
\end{table}

A set of reference grids provided by the MATPOWER library~\cite{pegase, matpower} is used during the experiments. The grids and their properties are summarized in Table~\ref{tab:Cases}. In what follows, the grid name will be suffixed by the number of considered transmission line contingencies.

\pgfplotstableread{
Name                Buses       Branches       Generators
PEGASE1354           1354           1991              260
PEGASE2869           2869           4582              510
PEGASE9241           9241          16049             1445
PEGASE13659         13659          20467             4092
}\grids
%ACTIVSg10k          10000          12706             1937

\begin{table}[!t]
	\renewcommand{\arraystretch}{1.3}
    	\caption{Properties of the benchmark power grids.}
	\label{tab:Cases}
	\centering
	\pgfplotstabletypeset[
	columns={Name,Buses,Branches,Generators},
	columns/Name/.style={column name=Name,string type,column type=l},
	every head row/.style={
		before row=\toprule,after row=\midrule},
	every last row/.style={
		after row=\bottomrule},
	]\grids
\end{table}

% %~\cite{CSCSdaint}
The experiments are performed on multicore Cray XC40 compute nodes of ``Piz Daint" at the Swiss National Supercomputing Centre, which consist of Intel  Xeon E5-2695 v4 at 2.10 GHz with 18 cores and 64 GB RAM. %interconnected with Dragonfly network topology.
%GCC 5.3.0 compiler, Cray MPICH/7.6.0 library, and
In all experiments we have used  Intel MKL implementation of BLAS and LAPACK (version 2017 update 3). Version 3.12.4 of \IPOPT{} \cite{IPOPT2006} and \PARDISO{} \cite{pardiso} of version 6.1.0 were used. The GPU accelerators installed at compute nodes are NVIDIA Tesla P100 with 16 GB memory using CUDA Toolkit version 8.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \section{Nonlinear Level Improvements}
% This section discusses various areas that have an impact on the convergence properties of the IPM method on the nonlinear level. These are initial point selection, convergence tolerance and selection of the barrier parameter update strategy.

% \subsection{Initial Point Seleciton Strategy \label{sec:WarmstartResults}}
% As discussed in section \ref{sec:Warmstart} on IPM warm start strategies, we experiment with various initial points for the SCOPF problem, knowing the base case solution and including additional variables and constraints corresponding to the contingency scenarios.
% %Convergence from poor starting points, in the IPM literature, is achieved by penalty merit functions to enforce progress toward the solution. However, a wise choice of the initial guess may significantly reduce the amount of iterations to convergence. Several strategies of the primal variables initialization are discussed below.

% The computationally simplest strategy is to set bounded control variables to the midpoint of their allowed range, or close to a bound if bounded only from one side, i.e. so called ``flat start''. Alternative strategies try to suggest approximations of the SCOPF problem solution based on the solution of simpler problem. As demonstrated in Figure~\ref{fig:itersx0}, the number of iterations until convergence may vary significantly with different starting points. We assume the following starting point choices: (i) local solutions of the PF equations for each contingency scenario, which satisfy the equality constraints but not necessarily the bounds on variables or the inequality constraints, (ii) solution of the OPF problem for the nominal case, which satisfy both the equality and inequality constraints (including the variable bounds) for the nominal case (iii) solution of local OPF for each contingency scenario, and finally, (iv) the solution of local SCOPF problems considering the nominal case and the contingency of the given scenario. The results in Figure~\ref{fig:itersx0} indicate, that a good choice is the solution of the nominal OPF problem. It provides convergence similar to more expensive approximations, such as local OPF or even local SCOPF with a single contingency, yet being cheaper to compute.
% The computation of the nominal OPF may be further improved by using the PF solution as an initial guess for the OPF problem computation and using relaxed convergence tolerances since we are not interested in the exact solution. Note that if the initial point does not strictly satisfy the variable bound constraints, \IPOPT{} enforces these by shifting the corresponding entries of the initial guess that do not satisfy this criterion in order to be sufficiently inside the bounds. This is necessary in order to be able to evaluate the logarithmic barrier function \eqref{eq:Barrier}, which is defined only for the points satisfying the bound constraints.

% \begin{figure}[ht!]
% 	\input{figures/fig_itersx0.tex}
% 	\vspace{-5mm}
% 	\caption{\label{fig:itersx0} Number of iterations until convergence for different initial guesses. Considering 10 contingency scenarios. %$\epsilon_{tol} = 10^{-2}$.
% 	}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Convergence Tolerance}
% %DISCUSSION OF THE IPM TOLERANCE vs. OBJECTIVE and INFEASIBILITY
% As discussed in section \ref{sec:Scaling}, the scaled optimality error is used to determine the convergence criteria. Very tight convergence tolerances might require performing extra IPM iterations, while not improving the objective value nor constraint violations. We have observed that the objective function value and infeasibility norms stop decreasing at tolerance $\epsilon_{tol} = 10^{-2}$. Trying to reach tighter tolerances has only negligible impact on the objective improvement, while requiring more iterations and rather unexpectedly deteriorating the constraints violations in order to improve the optimality. The optimizer stops prematurely for the tolerances $\epsilon_{tol} \leq 10^{-9}$ since the algorithm detects no improvement in the objective function value nor infeasibility norms. Table \ref{tab:Errors} displays influence of the tolerance on number of IPM iterations and the objective function value and constraint violations for the case PEGASE1354 with 100 contingencies. Nominal OPF used as the initial guess.
% %This indicates that the desired tolerances are too small for the current problem and there is indeed no significant improvement compared to less strict convergence tolerance.

% %TABLE SHOWING OBJECTIVE AND INFEASIBILITY FOR DECREASING TOLERANCES
% \begin{table} [!th]
% 	\renewcommand{\arraystretch}{1.3}
% 	\caption{Influence of the stopping tolerance $\epsilon_{tol}$ to the number of IPM iterations and the quality of the solution.}
% 	\label{tab:Errors}
% 	\centering
% 	\pgfplotstabletypeset[
% 	%columns={Tolerance,Iterations,Objective,BusPF,BranchPF,Bounds},
% 	columns={Tolerance,Iterations,Objective,BusPF,BranchPF},
% 	columns/Name/.style={column name=Name,string type,column type=l},
% 	every head row/.style={
% 		before row={
% 		    \toprule
% 			& & & \multicolumn{2}{c}{Constraint violations} \\
% 			\cmidrule(l{4pt}r{2pt}){4-5}
% 		},
% 		after row=\midrule,
% 	},
% 	every last row/.style={
% 		after row=\bottomrule},
% 	columns/Tolerance/.style  ={sci zerofill, precision=0,column name=\textbf{Tolerance}},
% 	columns/Objective/.style  ={zerofill, precision=3,column name=Objective (\$/h)},	
% 	%columns/Bounds/.style  ={column name=Variable Bounds},
% 	columns/BusPF/.style  ={sci,sci zerofill,precision=3,column name={Nodal balance}},
% 	columns/BranchPF/.style  ={sci zerofill,precision=2,column name={Line flow}},
% 	]{data/convergence.dat}
% \end{table}

% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Barrier Parameter Update Strategy}
% Adaptive vs. monotone (initial value, if warmstart show the trend with increasing NC)

% Number of iterations for various benchmarks, adaptive vs. monotone (with different starting values) + influence of the monotone $\mu_0$ for the warm start.

% \subsection{Scaling of the Problem}
% number of iterations for various benchmarks and scalings (none, gradient with different values, equilibration-based)

% \subsection{Effect of the linear system Solver}
% Include results from the matpower-opf paper. Discuss not only the performance but also number of iterations, discuss quality of the search direction and numerical errors.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Accuracy and Performance of the Distributed Solution \label{sec:schurResults}}
%\section{Parallel Solution of the KKT System \label{sec:schurResults}}
The most computationally expensive part of the optimization process for large-scale optimal control problems is the solution of the KKT system. Using a general direct sparse solver, that does not take into account the matrix structure, the solution of the KKT system consumes up to $99.99$\% of the overall run time, as demonstrated in Figure~\ref{fig:serial}. The other contributions from function evaluations (e.g., objective, Hessian of Lagrangian, or Jacobian of constraints), vector updates, or convergence criterion evaluation inside IPM, are orders of magnitude smaller. Reduction in the KKT solution time therefore significantly improves the overall run time.

\begin{figure}[!ht]
	\input{figures/fig_serial.tex}
	\caption{Overview of the \IPOPT{} components contributing to the overall time for a fixed number of IPM iterations, demonstrating the IPM bottleneck. \label{fig:serial}}
\end{figure}

% The comparison of different solution algorithms is not valid unless all of them make the optimization algorithm converge to the same optimal solution. The Schur complement based solution strategy is just a different way of solving the KKT linear system, so it does not change the convergence properties of the IPM. Nevertheless, due to the floating point arithmetics, the round-off errors may introduce significant contribution so that at some point the IPM with different linear system solution strategy might take different trajectory, but we have observed this only for very ill-conditioned linear system. The residuals for the KKT system solutions arising in PEGASE1354-100 benchmark are shown in figure \ref{fig:residual}. In order to improve robustness of the implementation, it is very important to use the iterative refinement in order to obtain highly accurate solutions. In \IPOPT{} algorithm, the iterative refinement (IR) is computed for the original, non-reduced, KKT system \eqref{eq:SCOPFhessian}. The figure \ref{fig:residual} presents residual of the first solution only, since the number of IR might vary between the two approaches. %and thus the presentation of the results w.r.t the x-axis would be difficult
%TODO: show number of IR for the direct and beltistos for the given benchmark PEGASE1354-100

%Residuals of the KKT linear system solve
% \begin{figure*}[!ht]
% 	\centering
% 	\begin{subfigure}[t]{0.5\textwidth}
% 		\centering
% 		\input{figures/fig_residuals118.tex}
% 		\caption{IEEE118-159 \label{fig:residualA}}
% 	\end{subfigure}%
% 	~ 
% 	\begin{subfigure}[t]{0.5\textwidth}
% 		\centering
% 		\input{figures/fig_residuals1354.tex}
% 		\caption{PEGASE1354-100 \label{fig:residualB}}
% 	\end{subfigure}
% 	\caption{Residuals of the KKT linear system solve using different solution approaches - direct solve and Schur Complement approach with and without elimination of the slack variables. No iterative refinement. (\BELTISTOS{}-aug needs more IRs, in Pardiso's case Ipopt asks for 1IR, for Schur usually more).  \label{fig:residuals}}
% \end{figure*}

% \begin{figure}[!ht]
% 	\centering
% 	\input{figures/fig_residuals1354.tex}
% 	\caption{Residuals of the KKT linear system solve.  \label{fig:residual}}
% 	%(No iterative refinement. \BELTISTOS{}-aug needs more IRs, in Pardiso's case Ipopt asks for 1IR, for Schur usually more).
% \end{figure}

% Figure~\ref{fig:objective} shows the convergence trajectory of the objective function and infeasibility norms for the PEGASE1354-100 benchmark using the direct factorization approach, as implemented in \PARDISO{} linear solver, and distributed \mbox{\BELTISTOS{}-$4$-aug} approach. The two approaches take the same trajectories during the optimization process and converge to the same solution.
% %The convergence process is shown in detail for two selected benchmarks in the Figure~\ref{fig:objective}. 
% Note the sudden changes in the infeasibility norms after iteration 60 that are the result of switching from one barrier sub-problem to the next one with decreased barrier parameter $\mu$. In Figure~\ref{fig:objective}, it is interesting to observe that even though the optimization problem is formulated as a minimization of the objective function, the objective function value is actually increasing at some IPM iteration horizons. This is a result of the fact that the optimization process is driven by satisfying the constraints with higher priority than improving the objective function value.
%{\color{red} Note that this is not neccesarily always the case, optimizers may take different trajectories due to ill-conditioning of the linear system (also, Schur ignores the intertia).}

% Convergence trajectory for the direct and schur approaches
% \begin{figure*}[!ht]
% 	\centering
% 	\begin{subfigure}[t]{0.5\textwidth}
% 		\centering
% 		\input{figures/fig_objective118.tex}
% 		\caption{IEEE118-159 \label{fig:objectiveA}}
% 	\end{subfigure}%
% 	~ 
% 	\begin{subfigure}[t]{0.5\textwidth}
% 		\centering
% 		\input{figures/fig_objective1354.tex}
% 		\caption{PEGASE1354-100 \label{fig:objectiveB}}
% 	\end{subfigure}
% 	\caption{Objective function value and infeasibility norms (primal and dual) over the iterations of the IPM with direct solution and distributed Schur solver. Tolerance fixed to $tol = 10^{-2}$. \label{fig:objective}}
% \end{figure*}

% \begin{figure}[!ht]
% 	\centering
% 	\input{figures/fig_objective1354.tex}
% 	\vspace{-0.3cm}
% 	\caption{Convergence trajectory for PEGASE1354-100 benchmark over the IPM iterations. Tolerance fixed to $tol = 10^{-2}$. \label{fig:objective}}
% \end{figure}

Figure~\ref{fig:parallel} demonstrates that by using the parallel \BELTISTOS{} solver with an increasing number of processes, the KKT solution time decreases and thus the overall run-time of the optimization is reduced accordingly. The performance of the \BELTISTOS{}-std approach is shown in Figure~\ref{fig:parallelSTD}. The single-process performance is several times slower than the ``Direct'' approach, but with increasing number of parallel processes the overall time scales down proportionally and outperforms the ``Direct'' approach. On the other hand, the single-process performance of the \BELTISTOS{}-aug approach, shown in Figure~\ref{fig:parallelAUG}, is almost two orders of magnitude faster than the ``Direct'' approach and it is possible to further decrease the solution time with additional parallel processes. 
%The detailed investigation of the performance differences between the two approaches is explored in the following section.

\begin{figure*}[!th]
	\centering
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\input{figures/fig_parallelSTD.tex}
		\caption{Standard ``backsolve" \label{fig:parallelSTD}}
	\end{subfigure}%
	~ 
	\begin{subfigure}[t]{0.5\textwidth}
		\centering
		\input{figures/fig_parallelAUG.tex}
		\caption{Incomplete factorization approach \label{fig:parallelAUG}}
	\end{subfigure}
	\caption{Overview of the \IPOPT{} components for PEGASE9241-256 benchmark, where ``Direct'' solver is compared to parallel \BELTISTOS{}-N algorithms with different Schur complement assembly approaches. \label{fig:parallel}}
	%Number of interior point iterations was fixed to 5.
\end{figure*}

Depending on the problem size, there is an upper limit to the number of parallel processes that are able to efficiently utilize available computing resources, since there are serial components in the IPM algorithm.
%the overall time stops scaling down with increasing number of parallel processes at some point
Such a situation can be observed in Figure~\ref{fig:parallelAUG}, where the function evaluations and other \IPOPT{} internal computations became as significant as the solution phase for 8 and more parallel processes. The effect of parallelization after this point will be deteriorated by these serial components. Another component influencing the parallel efficiency is assembly of the KKT system, which is performed solely at the master process and individual blocks need to be distributed to the available processes. The distribution step involves inherent interprocess communication and thus deteriorates the performance with increasing number of processes. The communication overhead becomes significant, especially if the workload per node is small, e.g., only a couple of scenarios per node.


% \begin{table}[!th]
% 	\centering
% 	\caption{\textbf{TODO: Update} Comparison of SCOPF optimization problem using \PARDISO{} and distributed Schur solver with 4 parallel processes. IPOPT runs until convergence with tolerance set to $10^{-2}$.}
% 	\label{tab:convergence}
% 	\input{tab_convergence.tex}
% \end{table}

% \begin{figure}[t!]
% 	\centering
% 	\input{figures/fig_residuals.tex}
% 	\caption{Residuals of the PEGASE9241-16 KKT system solution using \PARDISO{} and Schur solver with different sets of \PARDISO{} parameters. \label{fig:residuals}}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% \subsection{Node Level Parallelism}
% We investigate the behavior of the linear algebra presented in Section~\ref{sec:augmented} on multicore nodes. Figure~\ref{fig:schur} displays the average execution times to compute $BA^{-1}B^{\transpose}$ from \eqref{eq:SCform} on the XC40 node for different benchmarks using different numbers of CPU cores. The benchmarks contained 16 contingency scenarios each, while the average compute times per scenario are reported. For reference, we also show the average times of the \BELTISTOS{}-1-std ``backsolve" approach. Both approaches used \PARDISO{}, but each approach used different functionality of the software. We note that the augmented incomplete factorization times are orders of magnitude smaller than the ``backsolve'' times, especially with the large problems such as PEGASE9241 and PEGASE13659. Due to the extensive memory requirements for storing the RHS in the \mbox{\BELTISTOS{}-1-std} only its single-core execution is demonstrated.

% Figure~\ref{fig:schur} also reveals that the multithreaded augmented approach scales reasonably well with the number of threads. The observed speedup of the 16 threaded run over the single threaded case was $6.3\times$ for the smallest benchmark PEGASE1354, while for the largest case PEGASE13659 the speedup was only $2.6\times$ due to larger memory footprint and thus faster memory bandwidth saturation.
% \begin{figure}[ht!]
% 	\input{figures/fig_schur.tex}
% 	\caption{Comparison of the ``backsolve" \BELTISTOS{}-1-std vs. the augmented approach \BELTISTOS{}-1-aug-T with multiple threads. %to computing local Schur complement contributions $BA^{-1}B^{\transpose}$.
% 	\label{fig:schur}}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\subsection{Slack Variables Elimination}

The expected benefits of solving the reduced KKT system with eliminated slack variables compared to the unreduced system are savings both in terms of memory requirements for storing the sparse L factor of the LDL$^{\transpose}$ factorization, and possibly faster factorization and solution times due to smaller number of required floating point operations. The numerical evaluation and the results of solving the reduced system are summarized in Table~\ref{tab:slackElimination}.

The elimination of the slack variables from the KKT system reduces its dimension by approximately $30$\% with $13$\% fewer nonzeros in the system and up to $12$\% fewer nonzeros in the L factor, resulting in up to $28$\% memory savings for each of the diagonal blocks. The majority of the time in per-block computation is spent in factorization of the augmented matrix \eqref{eq:augmented}. Factorization time of the reduced system is improved up to $25$\% and the overall time of the local computation in Algorithm~\ref{alg:Schur} (steps~\ref{alg:SchurSCf1},~\ref{alg:SchurRHS}, and~\ref{alg:solve2}) is improved by up to $24$\%. Considering that the assembly of the local Schur complement is the main bottleneck and available memory on the compute nodes is limited, the achieved memory savings and time gain is significant, leading to more efficient and scalable code. 
%{\color{red} Discuss influence of the ordering during factorization and failure of metis5, poor results using Metis 4 for large-scale grids and somehow better MDO}
%We note that the benefit of solving the reduced system strongly depends on the quality of fill-in minimization reordering of the linear system performed during the factorization phase of the $A_i$. The factors of both the reduced and full $A_i$ have a similar number of nonzero entries for some linear system. The improvement in the number of nonzero entries in the L factor for the PEGASE13659 is only 0.12\%, as compared to 12\% improvement for the PEGASE1354, which is consequently reflected in the memory and time requirements.
%{\color{red} How do we argue than that the speedup is not the effect of better reordering but the reduced size of the block linear system? Wouldn't it be better to use better reordering algorithm rather than perform the slack elimination, which does not help that much??}
%{\color{red}(It's either that it does very good job before, or very poor job after the elimination)}
%Two variants of fill-in reordering algorithms (Metis 4 and Minimum degree ordering (MDO)) are presented in Table~\ref{tab:slackElimination} for the large scale networks, while smaller networks are shown for Metis 4 only. We can observe that using different fill-in minimizaiton reordering techniques, the benefit of slack variables elimination varies, and is especially visible in the time domain.

%THESE RESULTS ASSUME ELIMINATION OF ALL SLACK VARIABLES, ALTHOUGH IN PRACTICE IT IS NOT POSSIBLE TO ELIMINATE ALL OF THEM, SINCE AS THEY BECAME CLOSE TO 0 WE WOULD BE INVERTING MATRIX WITH SOME OF THE DIAG. ENTRIES 0 WHICH SERIOUSLY DETERIORATES THE PRECISION OF SUCH SOLVE. INSTEAD WE CAN ELIMINATE ONLY VARIABLES WHERE CORRESPONDING L_s IS GREATER THAN SOME THRESHOLD (E.G. 1E-8).

%https://tex.stackexchange.com/questions/9132/rounding-numbers-in-a-table-truncating-text-in-table
\begin{table}[!t]
	\centering
	%\caption{Comparison of per-block $A_i$ computation without and with slack variables elimination.}
	%\caption{Improvement rate of per-block $A_i$ computation considering elimination of the slack variables.}
	\caption{Improvement rate of solving the reduced KKT system with eliminated slack variables. Considering per-block $A_i$ computation.}
	\label{tab:slackElimination}
	\input{tab_elimination.tex}
\end{table}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\subsection{GPU Dense Linear Algebra}
% \subsection{GPU Acceleration}
% %Dense Schur system solved on single node - serial bottleneck
% %decrease serial time to minimum in order to retain scaling
% The bottleneck of the parallel Schur algorithm is the dense linear algebra associated with the global part of the solution in \eqref{eq:hessianPerm}, which is solved exclusively by a single process. The dense Schur system needs to be factorized and a forward-backward substitution needs to be performed with the computed factors, corresponding to steps~\ref{alg:schurF} and~\ref{alg:schurS} in Algorithm~\ref{alg:Schur}, respectively. GPU accelerated cuSolveDN library for dense linear systems is used to reduce the time of this serial component of the algorithm in order to increase parallel efficiency and further decrease overall time to solution. Table~\ref{tab:gpu} summarizes the dense linear algebra solution time, using the GPU accelerated library compared to the Intel MKL LAPACK implementation for CPU. N denotes size of the dense Schur complement, and the GPU related memory transfers are presented separately from the solution time.
% As a remark, the size of the dense Schur system is constant, independent on the number of considered contingencies for each grid. 
% We observed speedup of up to $30 \times$ using GPU for the largest grid, considering also the penalty of the memory transfers between CPU and GPU. The GPU acceleration is vital, since the improved sparse linear algebra reduces computational time to such extent that the dense computation times start to present significant contribution to the overall run time, especially for the large-scale power networks.
% \begin{table}[!ht]
% 	\centering
% 	\caption{Solution and memory transfer times [ms] of the dense Schur complement systems.}
% 	%Size of the matrix is denoted by N.
% 	\label{tab:gpu}
% 	\input{tab_gpu.tex}
% \end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\section{Large Scale Simulations}
\subsection{Performance Case Study}

% \begin{table}[!ht]
% 	\centering
% 	\renewcommand{\arraystretch}{1.3}
% 	\caption{Properties of the large-scale benchmarks.}
% 	\label{tab:benchmarks}
% 	\pgfplotstabletypeset[
% 	columns/Case/.style={column name={\textbf{Benchmark}},string type,column type=l},
% 	every head row/.style={
% 		before row=\toprule,after row=\midrule},
% 	every last row/.style={
% 		after row=\bottomrule},
% 	columns={Case, NC, Vars, Constr, Nrows},
% 	columns/NC/.style={column name={$\boldsymbol N_c$}},
% 	columns/Vars/.style={column name={\textbf{Variables}}},
% 	columns/Constr/.style={column name={\textbf{Constraints}}},
% 	columns/Nrows/.style={column name={\textbf{KKT size}}},
% 	]{data/benchmarks.dat}
% 	%PEGASE13659     128  3505014    8736256     17480822
% 	%PEGASE1354     2048  5548550    13701120    27404806
% 	%PEGASE9241      256  4734536    12948480    24670582
% 	%PEGASE9241      512  9466184    25896960    51797320
% \end{table} 

%%MEMORY REQUIREMENTS
% \begin{figure}[ht!]
% 	\input{memory.tex}
% 	\caption{Memory requirements for storing the symmetric upper-triangular part of the KKT system for the benchmark cases with growing number of contingencies. \label{fig:memory} }
% \end{figure}
We report on the strong scaling efficiency of the \BELTISTOS{}-aug solver on ``Piz Daint", using an increasing number of compute cores on the distributed memory compute nodes.  
The number of considered contingency scenarios was selected such that the problem does not exceed the memory limit of 64 GB available at each compute node since the current implementation requires assembly of the linear system on a single node with subsequent distribution of its parts to the remaining processes. 
%
%This memory limit turned out to be very restrictive since it did not allow us to solve arbitrarily large problems and demonstrate scaling up to very large number of compute cores. 
%
The largest instance of the solved problem contained up to $1.11 \cdot 10^7$ variables and $2.74 \cdot 10^7$ constraints. 
%The properties of the two large-scale benchmark problems are summarized in Table~\ref{tab:benchmarks}. Number of considered contingencies $N_c$, overall number of variables, constraints and size of the resulting KKT system are presented.

Figure~\ref{fig:scaling} shows the average wall time of the individual phases of the Algorithm~\ref{alg:Schur}, indicating also the ideal strong scaling. The algorithmic phases shown in the figure are: the initialization phase (\textit{init}), assembly of the Schur complement in steps~\ref{alg:SchurSCf1}--\ref{alg:SchurSCf2} (\textit{SC Assembly}), GPU accelerated Schur complement solution in steps~\ref{alg:schurF}--\ref{alg:schurS} (\textit{GPU Computation}), and solutions of the local parts of the system in steps~\ref{alg:solve1}--\ref{alg:solve2} (\textit{Local Solve}). The benchmarks were run with a single MPI process per node and each process contained 16 threads. %Figure~\ref{fig:scaling} also demonstrates speedups of the \BELTISTOS{}-aug solver compared to the serial direct factorization.

The \BELTISTOS{}-aug approach using a single process outperforms the sequential direct factorization by a factor of up to $40\times$ and $270\times$ for the two benchmarks, respectively. The observed speedup increased up to $500\times$ and $4200\times$, respectively, with an increasing number of distributed memory nodes. The significant speedup difference between the two benchmark cases may be attributed to nonsatisfactory performance of the serial direct factorization for the PEGASE9241-512 benchmark due to extensive fill-in. Although both KKT systems have similar size and number of nonzero entries, there is a factor of 13$\times$ difference between the factorization time of the two.
The speedups are expected to grow significantly for larger problems, but due to the restrictive memory at the ``Piz Daint" machine, it is not possible to demonstrate.
%
The \BELTISTOS{}-aug solution time scales reasonably up to $512$ cores at $32$ compute nodes, which in terms of workload translates to $16$ scenarios per node of PEGASE9241 or $128$ scenarios per node of PEGASE1354 benchmark. At this point, the initialization phase requires approximately the same time as the most expensive part of the algorithm, which is the computation of the local contributions to the Schur complement. Thus, the initialization phase is the inherent bottleneck of this approach and determines the scalability limits. We have decided not to attempt the implementation of fully distributed and parallel IPM framework since this was accomplished before, e.g. by PIPS-IPM \cite{CosminCurvature, pardiso}. The purpose was to show that more efficient implementation is possible by implementing sparse linear algebra routines which further improve intra-node performance compared to the previous work. The proposed method employs one additional Schur complement, chosen so that the sparsity of the KKT matrix is maintained. Consequently, the size of the linear system decreases and this allows for memory savings and increased computational performance.

\begin{figure}[t!]
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\input{figures/fig_scaling2.tex}
		\vspace{-0.5cm}
		\caption{PEGASE1354-4096}
	\end{subfigure}
	\hfill
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\input{figures/fig_scaling1.tex}
		\vspace{-0.5cm}
		\caption{PEGASE9241-512}
	\end{subfigure}%
	\caption{\label{fig:scaling} Strong scaling of the parallel \BELTISTOS{}-N-aug-16 solver and its components on two SCOPF benchmarks. Additionally, the speedup with respect to the serial ``Direct'' approach is shown.} 
	%Average solution time over multiple runs together with its ideal scaling is shown. The components contributing to the overall time are also presented, namely initialzation of the linear system system to the distributed environment, time to form the Schur complement, solution of the dense Schur system including assembly of the RHS, and the solutions of the local systems. 
%FACTORS THAT COULD CONTRIBUTE TO THE BIG DIFFERENCE IN THE PERFORMANCE OF THE TWO CASES (500 VS. 4K)
%1) Both KKT systems are of approx. same size with same number of KKT NNZ, what differs is size and number of the diagonal blocks.
%2) Hypothesis: What is the number of NNZ in the factors of the full KKT system? The pegase9k system takes 13x more compared to pegase1k using the direct solve; while the the difference for Schur-1 is only 2x. It is probably the case that direct for pegase9k fails to find good reordering and produces a lot of fill in
%3) wasn't it the case that the pegase9k system was refactorized due to the incorrect inertia?
\end{figure}

\begin{figure*}[t!]
	\centering
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\input{figures/fig_weak2.tex}
		\vspace{-0.5cm}
		\caption{PEGASE1354, 128 scenarios per node}
	\end{subfigure}
	~
	\begin{subfigure}[t]{0.49\textwidth}
		\centering
		\input{figures/fig_weak1.tex}
		\vspace{-0.5cm}
		\caption{PEGASE9241, 16 scenarios per node}
	\end{subfigure}%
	\caption{Weak scaling of the parallel \BELTISTOS{}-N-aug-16 solver and its components on two SCOPF benchmarks. Additionally, the parallel efficiency is shown.  \label{fig:scalingWeak}}
\end{figure*}

%\begin{figure}[ht!]
%	\input{iterations.tex}
%	\caption{Behavior of the parallel solver over the iteration horizon.}
%\end{figure}

%\begin{figure}[ht!]
%	\input{drosos.tex}
%	\caption{Behavior of the parallel solver over the iteration horizon.}
%\end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


==> 05Administration.tex <==
\chapter{Administration and Research Roadmap \label{chapter:Admin}}

This section summarizes a timeline of the work performed since the beginning of the PhD studies (09/2015), including the grades overview, TA duties, and a listing of the journal and conference publications. The document is concluded by presenting a schedule for conducting and completing the work in approximately 2020.

\begin{table}[h!]
\centering
\caption{Breadth requirement overview.}
\label{tab:courses}
\begin{tabular}{lllll}
\hline
Course                           & Grade & ECTS & Semester & Type  \\ \hline
Deterministic Methods            &   8  & 4    & Fall 15/16    & MSc X \\
Numerical Algorithms             &  8.5  & 2    & Fall 15/16   & MSc X \\
Stochastic Methods               &  8.5   & 4    & Spring 15/16  & MSc X \\
Introduction to Doctoral Studies &  pass    & 2    & Spring 15/16  & Ph.D.   \\ \hline
Research Prospectus &  pass    & -    & Dec 2016  & Ph.D.   \\ \hline
 \hline
\end{tabular}
\end{table}

\begin{table}[h!]
\centering
\caption{Courses served as a teaching assistant.}
\label{tab:ta}
\begin{tabular}{lllll}
\hline
Course                               & Instructor             & Program & Semester  \\ \hline
High-Performance Computing           &  Schenk Olaf           & MSc CS    & Fall  15/16  \\
Node-Level Performance Engineering   &  Wellein G., Hager G.  & MSc CS    & Spring 15/16  \\
CSCS-USI Summer school               &  CSCS staff \& USI           &    PhD      & Summer '16  \\
Numerical Computing                  &  Schenk Olaf           & BSc       & Fall  16/17 \\
Node-Level Performance Engineering   &  Wellein G., Hager G.  & MSc CS    & Spring  16/17 \\
Bachelor project                     &  Mehdi Jazayeri           & BSc    & Spring  16/17  \\
CSCS-USI Summer school               &  CSCS staff \& USI           &    -      & Summer '17  \\
High-Performance Computing           &  Schenk Olaf           & MSc CS    & Fall  17/18  \\
Software Atelier: Supercomputing           &  Schenk Olaf           & MSc CS    & Spring  17/18  \\
High-Performance Computing           &  Schenk Olaf           & MSc CS    & Fall  18/19  \\ \hline
 \hline
\end{tabular}
\end{table}

\begin{table}[h!]
\centering
\caption{Publications.}
\label{tab:journals}
\begin{tabular}{l p{11cm}}
ACM TOMS  & J. Kardos, D. Kourounis, O. Schenk, R. Zimmerman, \textit{An evaluation of interior point frameworks and variable formulations for large-scale optimal power flow problems}, Under revision\\
IEEE PES & J. Kardos, D. Kourounis, O. Schenk, \textit{Two-Level Parallel Augmented Schur Complement Interior Point Algorithms for the Solution of Security Constrained Optimal Power Flow Problems}, Under revision.\\
SBAC-PAD &  F. Verbosio, J. Kardos, M. Bianco, O. Schenk, \textit{Highly Scalable Stencil-based Matrix-free Stochastic Estimator for the Diagonal of the Inverse} in 9th Workshop on Applications for Multi-Core Architectures, September 24-27, 2018 ENS Lyon, Lyon, France, 30th IEEE International Symposium on Computer, Architecture and High Performance Computing (SBAC-PAD 2018), September 24-27, 2018, Ecole Normale Superieure, Lyon, France  \\
Tech Report  & J. Kardos, D. Kourounis, O. Schenk, R. Zimmerman, \textit{Complete results for a numerical evaluation of interior point solvers for large-scale optimal power flow problems}. Eprint arXiv:1807.03964 (2018) \\
% Tech report  & J.Kardos, \textit{Evaluating realistic tsunami simulations with SWE model on GPU-enabled clusters}. Universit\'a della Svizzera italiana, June 2013. Report number USI-INF-TR-2013-03.\\
\hline \hline
\end{tabular}
\end{table}

\begin{table}[h!]
\centering
\caption{Conference presentations.}
\label{tab:conferences}
\bgroup
\def\arraystretch{2.5}
\begin{tabular}{l l}
\makecell[cl]{SCCER-FURIES\\ Lausanne}  &  \makecell[cl]{Toward the Next Generation of Multiperiod and Security Constrained\\ Optimization (Talk)}\\ 
\makecell[cl]{PASC18\\  Basel} & \makecell[cl]{A Distributed Parallel Approach for Large Scale Optimal Power Flow\\ with Security Constraints (Poster)} \\ 
\makecell[cl]{SIAM PP18\\ Tokyo} & \makecell[cl]{Security Constrained Optimization of Large-Scale Energy Systems\\ (Minisymposia presentation)} \\
\makecell[cl]{PASC16\\  Lausanne} & \makecell[cl]{Using GridTools library to implement Preconditioned Conjugate\\ Gradient Krylov solver (Minisymposia presentation)}  \\
\makecell[cl]{SIAM PP16\\  Paris} & \makecell[cl]{Interior-Point Stochastic Approximation Method on Massively\\ Parallel Architectures (Poster)} \\
\makecell[cl]{PASC14\\ Z\" urich} & \makecell[cl]{Evaluating Realistic Tsunami Simulations with SWE Model on \\GPU-enabled Clusters (Poster)} \\
\hline \hline
%Swiss Numerics Days  (Minisymposia presentation) & Security Constrained Optimization of Large-Scale Energy Systems. \\
\end{tabular}
\egroup
\end{table}

%\section{Reduced Space IPM}
The remaining study will be focused on investigation of the performance and convergence behavior of the reduced space IPM. The tasks to be performed and questions to be answered are the following:
(i) implement the reduced space solution approach and the constraint lumping techniques;
(ii) run the benchmarks to measure the performance and compare it with the parallel KKT solution approach;
%(iii) determine how significant are the serial components of the reduced space approach and to which extent the overall parallel efficiency could be degraded,
(iii) will be convergence of the quasi-Newton method satisfactory in the reduced space approach? (iv) Can we achieve significant computational complexity reduction using the constraint lumping lumping technique? Will it influence the convergence rate?

%\section{Application for the Parallel KKT Solver}
The remaining time of the PhD studies will be also focused on finding an application for the existing implementation of the parallel structure exploiting solver. There are couple of possible scenarios. First, the application can be found within the SCCER-FURIES project. Dr. Turhan Demiray is working on a flexible, modular, and computationally efficient transient simulation framework for the electric power grid problems. The structure of the linear systems resulting from the time discretization is appropriate for the parallel Schur complement decomposition scheme.
Another possibility of applying the parallel KKT solver is the ARPA-E Grid Optimization Competition. \footnote{https://gocompetition.energy.gov} The competition is aiming to support the development of transformational ways to solve power flow optimization problems across a wide range of operating conditions. The participation in the competition will be a joint initiative with the Lawrence Livermore National Laboratory (LLNL) group of Cosmin Petra. The goal of the project is not only solving extreme-scale problems on HPC clusters, but a holistic approach to the problem, including contingency screening procedure and smart ways of dealing with non-smooth aspects of the real-life SCOPF problem formulation.
Another possibility of the application is the industrial partner Neplan, who might be interested in the reduced space IPM for the solution of the OPF and SCOPF problems, especially if the constraint lumping techniques will achieve significant computational complexity savings and the solution of these problems can be performed on a standard workstation.

%\section{Augmented Lagrangian}
A widespread alternative to the IPMs used in practice are augmented Lagrangian methods. In particular, a variant of the standard augmented Lagrangian method that uses partial updates known as the alternating direction method of multipliers gained a lot of  attention in the context of parallel computing. The dissertation might be extended by the augmented Lagrangian method study and implementation that will be investigated during the summer '19 internship at the LLNL under supervision of Cosmin Petra.

% Cosmin Petra has developed HiOp\footnote{https://github.com/llnl/hiop} optimization framework \cite{hiop}. HiOp is a lightweight HPC solver that leverages application's existing data parallelism to parallelize the optimization iterations by using specialized linear algebra kernels. It implements reduced-space quasi-Newton algorithm in IPOPT for problems where number of variables is large but number of non-trivial constraints (excluding the bound constraints) is small. 





==> figures/tab_convergence.tex <==
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Iterations}}                            & \multicolumn{2}{c}{\textbf{Objective} }  \\ \cmidrule(l{2pt}r{4pt}){2-3} \cmidrule(l{4pt}r{2pt}){4-5}
\multicolumn{1}{c}{\textbf{Benchmark}}           & \multicolumn{1}{c}{\textbf{\scriptsize{Pardiso}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Schur-4}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Pardiso}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Schur-4}}} \\ \midrule
\multicolumn{1}{l}{\scriptsize{IEEE118-32}}     &    47   &  30   &  1.3070216e+05 & 1.3070216e+05\\ 
\multicolumn{1}{l}{\scriptsize{IEEE118-64}}     &    48   &  49   &  1.3199916e+05 & 1.3199916e+05\\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-32}}  &    88   &  44   &  7.4076812e+04 & 7.4076812e+04\\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-64}}  &    83   &  37   &  7.4087249e+04 & 7.4129903e+04\\ 
\multicolumn{1}{l}{\scriptsize{PEGASE9241-16}}  &  150+   &  44   &  infeasible & 3.1596674e+05\\ 
\bottomrule
\end{tabular}

==> figures/tab_elimination.tex <==
%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r r G r r G}
\toprule
& \multicolumn{3}{c}{\textbf{Peak Memory [GB]} }  & \multicolumn{3}{c}{\textbf{Solution Time [$s$]} }\\ 
\cmidrule(l{2pt}r{4pt}){2-4} \cmidrule(l{4pt}r{2pt}){5-7}
\multicolumn{1}{c}{\textbf{Benchmark}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}} \\ \midrule
%
\multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
\multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
\multicolumn{1}{l}{\scriptsize{ACTIVSg10k}} & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
\multicolumn{1}{l}{\scriptsize{PEGASE13659}} & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
\bottomrule
\end{tabular}


%%%% table with Nrows, Memory and Time statistic
% %G is a custom column with gray background, defined in preamble
% \begin{tabular}{l r r G r r G r r G}
% \toprule
% & \multicolumn{3}{c}{\textbf{Nrows $A_i$}}  & \multicolumn{3}{c}{\textbf{Peak Memory [GB]} }  & \multicolumn{3}{c}{\textbf{Solution Time [$s$]} }\\ 
% \cmidrule(l{2pt}r{4pt}){2-4} \cmidrule(l{4pt}r{2pt}){5-7} \cmidrule(l{4pt}r{2pt}){8-10}
% \multicolumn{1}{c}{\textbf{Benchmark}}           & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
% & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
% & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}} \\ \midrule
% %
% \multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 13,899 & 9,971 & 28.65 & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 30,823 & 21,659 & 29.73 & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 104,049 & 71,951 & 30.85 & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k}} & 94,697 & 69,285 & 26.84 & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659}} & 144,687 & 103,753 & 28.29 & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
% \bottomrule
% \end{tabular}

%%%%Full set of results. Above we show only the better of the MDO/Metis variants and do not further discuss this in the text.
% \multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 13,899 & 9,971 & 28.65 & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 30,823 & 21,659 & 29.73 & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 104,049 & 71,951 & 30.85 & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k-Metis4}} & 94,697 & 69,285 & 26.84 & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k-MDO}} & 94,697 & 69,285 & 26.84 & 0.109 & 0.101 & 7.29 & 0.899 & 0.848 & 5.73 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-Metis4}} & 144,687 & 103,753 & 28.29 & 0.326 & 0.316 & 3.07 & 2.029 & 2.256 & -11.22 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-MDO}} & 144,687 & 103,753 & 28.29 & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\

==> figures/tab_gpu.tex <==
%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r r r r G}
\toprule
& \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CPU}}   & \multicolumn{2}{c}{\textbf{GPU} } & \multicolumn{1}{c}{}  \\ \cmidrule(l{2pt}r{4pt}){3-3} \cmidrule(l{4pt}r{2pt}){4-5}

\multicolumn{1}{c}{\textbf{Benchmark}}    & \multicolumn{1}{c}{\textbf{N}}       & \multicolumn{1}{c}{\textbf{\scriptsize{Solution}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Solution}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Memory}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Speedup}}}\\ \midrule
\multicolumn{1}{l}{\scriptsize{PEGASE1354}}  &    518   &  19.7   &  13.1 & 0.8 & 1.41 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE2869}}  &    1,018   &  131.1   &  21.2 & 1.4 & 5.80 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE9241}}  &  2,888   &  416.3  &  50.7 & 7.4 & 7.16 \\ 
\multicolumn{1}{l}{\scriptsize{ACTIVSg10k}}  &  3,663   &  925.9  &  71.5 & 11.3 & 11.18 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE13659}}  &  8,182   &  8,641.0  &  231.0 & 54.0 & 30.33 \\ 
\bottomrule
\end{tabular}


==> figures/tab_inexactIters.tex <==
%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r G r G}
\toprule
& \multicolumn{2}{c}{\textbf{Iterations} }  & \multicolumn{2}{c}{\textbf{Solution Time [$s$]} }\\ 
\cmidrule(l{2pt}r{4pt}){2-3} \cmidrule(l{4pt}r{2pt}){4-5}
\multicolumn{1}{c}{\textbf{Benchmark}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Exact Newton}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Quasi-Newton}}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Exact Newton}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Quasi-Newton}}} \\ \midrule
%
%\multicolumn{1}{l}{\scriptsize{PEGASE1354-5}}   & 18 & 290  & 10.373  & 61.953  \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-10}}  & 29 & 291  & 34.816  & 256.532  \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-15}}  & 22 & 214  & 56.786  & 223.452  \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-20}}  & 29 & 360  & 98.594  & 733.369  \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-5}}  & 31 & 108  & 76.108  & 1184.892  \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-10}} & 46 & 184  & 519.18  & 5646.728  \\ 
\bottomrule
\end{tabular}

==> figures/tab_inexactItersX0.tex <==
%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r G r G r G}
\toprule
& \multicolumn{2}{c}{\textbf{Warm start} }  & \multicolumn{2}{c}{\textbf{Flat start} }  & \multicolumn{2}{c}{\textbf{Rel. increase} }\\ 
\cmidrule(l{2pt}r{4pt}){2-3} \cmidrule(l{4pt}r{2pt}){4-5} \cmidrule(l{4pt}r{2pt}){6-7}
\multicolumn{1}{c}{\textbf{Benchmark}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Exact}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Quasi-Newton}}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Exact}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Quasi-Newton}}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Exact}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Quasi-Newton}}} \\ \midrule
%
\multicolumn{1}{l}{\scriptsize{PEGASE1354 }}  & 16 & 54  & 25  & 228  & 0.56 & 3.22 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE13659}}  & 21 & 43  & 56  & 300  & 1.67 & 5.98 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE2869 }}  & 26 & 68  & 29  & 201  & 0.12 & 1.96 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE3375 }}  & 16 & 134 & 35  & 197  & 1.19 & 0.47 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE9241 }}  & 21 & 76  & 63  & 275  & 2.00 & 2.62 \\ 
\multicolumn{1}{l}{\scriptsize{ACTIVSg10k }}  & 18 & 49  & 168 & 242  & 8.33 & 3.94 \\ 
\bottomrule
\end{tabular}

==> tab_convergence.tex <==
\begin{tabular}{lrrrr}
\toprule
& \multicolumn{2}{c}{\textbf{Iterations}}                            & \multicolumn{2}{c}{\textbf{Objective} }  \\ \cmidrule(l{2pt}r{4pt}){2-3} \cmidrule(l{4pt}r{2pt}){4-5}
\multicolumn{1}{c}{\textbf{Benchmark}}           & \multicolumn{1}{c}{\textbf{\scriptsize{Pardiso}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Schur-4}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Pardiso}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Schur-4}}} \\ \midrule
\multicolumn{1}{l}{\scriptsize{IEEE118-32}}     &    47   &  30   &  1.3070216e+05 & 1.3070216e+05\\ 
\multicolumn{1}{l}{\scriptsize{IEEE118-64}}     &    48   &  49   &  1.3199916e+05 & 1.3199916e+05\\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-32}}  &    88   &  44   &  7.4076812e+04 & 7.4076812e+04\\ 
\multicolumn{1}{l}{\scriptsize{PEGASE1354-64}}  &    83   &  37   &  7.4087249e+04 & 7.4129903e+04\\ 
\multicolumn{1}{l}{\scriptsize{PEGASE9241-16}}  &  150+   &  44   &  infeasible & 3.1596674e+05\\ 
\bottomrule
\end{tabular}

==> tab_elimination.tex <==
%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r r G r r G}
\toprule
& \multicolumn{3}{c}{\textbf{Peak Memory [GB]} }  & \multicolumn{3}{c}{\textbf{Solution Time [$s$]} }\\ 
\cmidrule(l{2pt}r{4pt}){2-4} \cmidrule(l{4pt}r{2pt}){5-7}
\multicolumn{1}{c}{\textbf{Benchmark}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
& \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}} \\ \midrule
%
\multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
\multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k}} & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659}} & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
\bottomrule
\end{tabular}


%%%% table with Nrows, Memory and Time statistic
% %G is a custom column with gray background, defined in preamble
% \begin{tabular}{l r r G r r G r r G}
% \toprule
% & \multicolumn{3}{c}{\textbf{Nrows $A_i$}}  & \multicolumn{3}{c}{\textbf{Peak Memory [GB]} }  & \multicolumn{3}{c}{\textbf{Solution Time [$s$]} }\\ 
% \cmidrule(l{2pt}r{4pt}){2-4} \cmidrule(l{4pt}r{2pt}){5-7} \cmidrule(l{4pt}r{2pt}){8-10}
% \multicolumn{1}{c}{\textbf{Benchmark}}           & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
% & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}}
% & \multicolumn{1}{c}{\textbf{\scriptsize{Before}}} & \multicolumn{1}{c}{\textbf{\scriptsize{After}}} & \multicolumn{1}{c}{\textbf{\scriptsize{\%}}} \\ \midrule
% %
% \multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 13,899 & 9,971 & 28.65 & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 30,823 & 21,659 & 29.73 & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 104,049 & 71,951 & 30.85 & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k}} & 94,697 & 69,285 & 26.84 & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659}} & 144,687 & 103,753 & 28.29 & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\
% \bottomrule
% \end{tabular}

%%%%Full set of results. Above we show only the better of the MDO/Metis variants and do not further discuss this in the text.
% \multicolumn{1}{l}{\scriptsize{PEGASE1354}} & 13,899 & 9,971 & 28.65 & 0.010 & 0.007 & 28.12 & 0.027 & 0.020 & 23.88 \\ 
% \multicolumn{1}{l}{\scriptsize{PEGASE2869}} & 30,823 & 21,659 & 29.73 & 0.023 & 0.017 & 28.57 & 0.066 & 0.052 & 21.90 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE9241}} & 104,049 & 71,951 & 30.85 & 0.081 & 0.066 & 19.20 & 0.380 & 0.290 & 23.74 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k-Metis4}} & 94,697 & 69,285 & 26.84 & 0.102 & 0.093 & 8.16 & 0.529 & 0.468 & 11.52 \\
% \multicolumn{1}{l}{\scriptsize{ACTIVSg10k-MDO}} & 94,697 & 69,285 & 26.84 & 0.109 & 0.101 & 7.29 & 0.899 & 0.848 & 5.73 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-Metis4}} & 144,687 & 103,753 & 28.29 & 0.326 & 0.316 & 3.07 & 2.029 & 2.256 & -11.22 \\
% \multicolumn{1}{l}{\scriptsize{PEGASE13659-MDO}} & 144,687 & 103,753 & 28.29 & 0.331 & 0.318 & 3.98 & 1.938 & 1.855 & 4.29 \\

==> tab_gpu.tex <==
%G is a custom column with gray background, defined in preamble
\begin{tabular}{l r r r r G}
\toprule
& \multicolumn{1}{c}{} & \multicolumn{1}{c}{\textbf{CPU}}   & \multicolumn{2}{c}{\textbf{GPU} } & \multicolumn{1}{c}{}  \\ \cmidrule(l{2pt}r{4pt}){3-3} \cmidrule(l{4pt}r{2pt}){4-5}

\multicolumn{1}{c}{\textbf{Benchmark}}    & \multicolumn{1}{c}{\textbf{N}}       & \multicolumn{1}{c}{\textbf{\scriptsize{Solution}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Solution}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Memory}}} & \multicolumn{1}{c}{\textbf{\scriptsize{Speedup}}}\\ \midrule
\multicolumn{1}{l}{\scriptsize{PEGASE1354}}  &    518   &  19.7   &  13.1 & 0.8 & 1.41 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE2869}}  &    1,018   &  131.1   &  21.2 & 1.4 & 5.80 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE9241}}  &  2,888   &  416.3  &  50.7 & 7.4 & 7.16 \\ 
\multicolumn{1}{l}{\scriptsize{ACTIVSg10k}}  &  3,663   &  925.9  &  71.5 & 11.3 & 11.18 \\ 
\multicolumn{1}{l}{\scriptsize{PEGASE13659}}  &  8,182   &  8,641.0  &  231.0 & 54.0 & 30.33 \\ 
\bottomrule
\end{tabular}

